Asymptotic Statistical Analysis of $f$-divergence GAN

Generative Adversarial Networks (GANs) have achieved great success in data generation. However, its statistical properties are not fully understood. In this paper, we consider the statistical behavior of the general $f$-divergence formulation of GAN, which includes the Kullback--Leibler divergence that is closely related to the maximum likelihood principle. We show that for parametric generative models that are correctly specified, all $f$-divergence GANs with the same discriminator classes are asymptotically equivalent under suitable regularity conditions. Moreover, with an appropriately chosen local discriminator, they become equivalent to the maximum likelihood estimate asymptotically. For generative models that are misspecified, GANs with different $f$-divergences {converge to different estimators}, and thus cannot be directly compared. However, it is shown that for some commonly used $f$-divergences, the original $f$-GAN is not optimal in that one can achieve a smaller asymptotic variance when the discriminator training in the original $f$-GAN formulation is replaced by logistic regression. The resulting estimation method is referred to as Adversarial Gradient Estimation (AGE). Empirical studies are provided to support the theory and to demonstrate the advantage of AGE over the original $f$-GANs under model misspecification.

==> parts/proof.tex <==
\section{Proofs in Section \ref{sec:method}}\label{app:pf_grad}

The proof technique is inspired by that of CFG-GAN \cite{Johnson2019AFO}.
Given a differentiable vector function $g(x):\mathbb{R}^k\to\mathbb{R}^k$, we use $\nabla\cdot g(x)$ to denote its divergence, defined as 
$$\nabla\cdot g(x):=\sum_{j=1}^k\frac{\partial[g(x)]_j}{\partial[x]_j},$$ 
where $[x]_j$ denotes the $j$-th component of $x$. We know that $\int\nabla\cdot g(x)dx=0$ for all vector function $g(x)$ such that $g(\infty) = 0$. Given a matrix function $w(x)=(w_1(x),\dots,w_l(x)):\mathbb{R}^k\to\mathbb{R}^{k\times l}$ where each $w_i(x)$, for $i=1\dots,l$, is a $k$-dimensional differentiable vector function, its divergence is defined as $\nabla\cdot w(x)=(\nabla\cdot w_1(x),\dots,\nabla\cdot w_l(x))^\top$.

To prove Theorem \ref{thm:grad}, we need the following lemma.
\begin{lemma}\label{lem:pf_grad}
Using the definitions in Theorem \ref{thm:grad}, we have 
\begin{equation}
\nabla_\theta p_\theta(x) = -g_\theta(x)^\top \nabla_x p_\theta(x) - p_\theta(x)\nabla\cdot g_\theta(x),\label{eq:grad_pgen}
\end{equation}
for all $x\in\cX$, where $g_\theta(G_\theta(z))=\nabla_\theta G_\theta(z)$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:pf_grad}]
Let $d_\theta$ be the dimension of parameter $\theta$. 
To simplify the notation, let $X=G_\theta(Z)\in\cX$ and $p$ be the probability density of $X$. For each $i=1,\dots,d_\theta$, let $\Delta=\delta e_i$ where $e_i$ is a $d_\theta$-dimensional unit vector whose $i$-th component is one and all the others are zero, and $\delta$ is a small scalar. Let $X'=G_{\theta+\Delta}(Z)$ and $\delta$ be such that $X'$ is a random variable transformed from $X$ by $X'=X+ g(X) \Delta + o(\delta)$ where $g(X)\in\mathbb{R}^{d\times l}$. Let $p'$ be the probability density of $X'$. For an arbitrary $x'\in\cX$, let $x'=x+g(x)\Delta+o(\delta)$. Then we have
\begin{align}
p'(x')&=p(x)|\det(dx'/dx)|^{-1}\nonumber\\
&=p(x)|\det(\id_d+\nabla g(x)\Delta+o(\delta))|^{-1}\nonumber\\
&=p(x)(1+\Delta^\top\nabla\cdot g(x)+o(\delta))^{-1}\label{eq:l0}\\ %check
&=p(x)(1-\Delta^\top\nabla\cdot g(x)+o(\delta))\label{eq:l1}\\
&=p(x)-\Delta^\top p(x')\nabla\cdot g(x') +o(\delta)\label{eq:l2}\\
&=p(x')-\Delta^\top g(x')^\top\cdot\nabla p(x') - \Delta^\top p(x')\nabla\cdot g(x') +o(\delta).\label{eq:l3}
\end{align}
The first two equalities use the multivariate change of variables formula for probability densities. (\ref{eq:l0}) uses the definition of determinant with terms explicitly expanded up to $O(\delta)$. (\ref{eq:l1}) uses the Taylor expansion of $(1+\gamma)^{-1}=1-\gamma+o(\gamma)$ with $\gamma=\Delta^\top\nabla\cdot g(x)$. (\ref{eq:l2}) follows from $p(x')=p(x)+o(1)$ and $\nabla\cdot g(x')=\nabla\cdot g(x)+o(1)$. (\ref{eq:l3}) is due to $p(x)=p(x')-(x'-x)^\top\nabla p(x')+o(\delta)$. 
Since $x'\in\cX$ is arbitrary, above implies that
\begin{eqnarray*}
p'(x)=p(x)-\Delta^\top g(x)^\top\nabla p(x)-\Delta^\top p(x)\nabla\cdot g(x) + o(\delta)
\end{eqnarray*}
for all $x\in\mathbb{R}^d$ and $i=1,\dots,d_\theta$, which leads to (\ref{eq:grad_pgen}) by taking $\delta\to0$, setting $g(x)=g_\theta(x)$, and noting that $p=p_\theta$ as both are the density of $G_\theta(Z)$ and $p'=p_{\theta+\Delta}$ as both are the density of $G_{\theta+\Delta}(Z)$. 
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:grad}]
Rewrite the objective (\ref{eq:obj}) as $L(\theta)=\int\ell(p_*(x),p_\theta(x))dx$ where $\ell$ denotes the integrands in definition (\ref{eq:f_div}).
Let $\ell'_2(p_*,p_\theta)=\partial\ell(p_*,p_\theta)/\partial p_\theta$.
Using the chain rule and Lemma \ref{lem:pf_grad}, we have 
\begin{align}
\nabla_\theta\ell(p_*(x),p_\theta(x))&=\ell'_2(p_*(x),p_\theta(x))\nabla_\theta p_\theta(x)\nonumber\\
&= \ell'_2(p_*(x),p_\theta(x))\big[-g_\theta(x)^\top\nabla_x p_\theta(x) - p_\theta(x)\nabla\cdot g_\theta(x)\big]\nonumber\\
&= p_\theta(x)g_\theta(x)^\top \nabla_x \ell'_2(p_*(x),p_\theta(x)) - \nabla_x\cdot\big[\ell'_2(p_*(x),p_\theta(x))p_\theta(x)g_\theta(x)\big],\label{eq:grad_int}
\end{align}
where the third equality is obtained by applying the product rule as follows
\begin{align*}
\nabla_x\cdot\left[\ell'_2(p_*(x),p_\theta(x))p_\theta(x)g_\theta(x)\right]&=\ell'_2(p_*(x),p_\theta(x))p_\theta(x)\nabla\cdot g_\theta(x) \\
&\ + \ell'_2(p_*(x),p_\theta(x))g_\theta(x)^\top \nabla_x p_\theta(x) \\
&\ + p_\theta(x)g_\theta(x)^\top \nabla_x \ell'_2(p_*(x),p_\theta(x)).
\end{align*}
By integrating (\ref{eq:grad_int}) over $x$ and by using the fact that $\int\nabla\cdot f(x)dx=\mathbf{0}$ with $f(x)=\ell'_2(p_*(x),p_\theta(x))p_\theta(x)g_\theta(x)$, we have
\begin{eqnarray*}
\nabla_\theta L(\theta,\phi) = \int\nabla_\theta\ell(p_*(x),p_\theta(x))dx=\int p_\theta(x) g_\theta(x)^\top \nabla_x \ell'_2(p_*(x),p_\theta(x))dx.
\end{eqnarray*}
According to the definition (\ref{eq:f_div}) of $f$-divergences and by noting the fact that $r(x)=e^{D^*(x)}$, we have  
\begin{eqnarray}\label{eq:lll}
\nabla_x \ell'_2(p_*(x),p_\theta(x))=f''\bigg(\frac{1}{r(x)}\bigg)\nabla_x \frac{1}{r(x)}=f''\bigg(\frac{1}{r(x)}\bigg)\frac{1}{r(x)}\nabla_x D^*(x).
\end{eqnarray}
Further by reparametrization, we obtain
\begin{align*}
\nabla_\theta L(\theta,\phi) &= -\mathbb{E}_{X\sim p_\theta(x)}\big[s^*(X)g_\theta(X)^\top \nabla_x D^*(x)\big]\\
&=-\mathbb{E}_{Z\sim p_z(z)}\big[s^*(G_\theta(Z))\nabla_\theta G_\theta(Z)^\top \nabla_x D^*(G_\theta(Z))\big],
\end{align*}
which completes the proof. 
\end{proof}




\section{Proofs in Section \ref{sec:theory}}

\subsection{Preliminaries}

This section presents some preliminary notions and lemmas which will be used in proofs.

\begin{definition}[Bracketing covering number \cite{geer2000empirical}]\label{def:cover_num}
	Consider a function class $\cG=\{g(x)\}$ and a probability measure $\mu$ defined on $\cX$. Given any positive number $\delta>0$. Let $N_{1,B}(\delta,\cG,\mu)$ be the smallest value of $N$ for which there exist pairs of functions $\{[g_j^L,g_j^U]\}_{j=1}^N$ such that $\int |g_j^L(x)-g_j^U(x)|d\mu\leq\delta$ for all $j=1,\dots,N$, and such that for each $g\in\cG$, there is a $j=j(g)\in\{1,\dots,N\}$ such that $g_j^L\leq g\leq g_j^U$. Then $N_{1,B}(\delta,\cG,\mu)$ is called the $\delta$-bracketing covering number of $\cG$.
\end{definition}


\begin{lemma}\label{lem:conv_density}
	Let $\mu_n$ and $\mu$ be a sequence of measures on probability space $(\cX,\Sigma)$ with densities $p_n(x)$ and $p(x)$. Given any compact subset $K$ of $\cX$. Suppose $p_n$ is uniformly bounded and Lipschitz on $K$ ($*$). If $H^2(\mu_n,\mu)\pto0$, then $\sup_{x\in K}|p_n(x)-p(x)|\pto0$ as $n\to\infty$, where $H(q_1,q_2)=\left(\int(q_1^{1/2}-q_2^{1/2})dxdz/2\right)^{1/2}$ denotes the Hellinger distance between two distributions with densities $q_1$ and $q_2$.
\end{lemma}
\begin{proof}
Note that assumptions in ($*$) satisfy the requirements in the Arzel\`a-Ascoli theorem. Thus, for each subsequence of $p_n$, there is a further subsequence $p_{n_m}$ which converges uniformly on compact set $K$, i.e., for some $p_0$ as $m\to\infty$ we have
\begin{equation*}
	\sup_{x\in K}|p_{n_m}(x)-p_0(x)|\to0.
\end{equation*}

By Scheff\'e's Theorem we have $H(p_{n_m},p_0)\to0$. On the other hand we have $H(p_{n_m},p)\pto0$. By triangle inequality,
\begin{equation*}
	H(p,p_0)\leq H(p_{n_m},p_0)+H(p_{n_m},p)\pto0.
\end{equation*}
Since the inequality holds for all $m$ and the LHS is deterministic, we have $H(p,p_0)=0$, which implies $p=p_0$, a.e. wrt the Lebesgue measure. Hence we have
\begin{equation*}
	\sup_{x\in K}|p_{n_m}(x)-p(x)|\to0,\ a.e.
\end{equation*}
Then by \cite[Theorem 2.3.2]{durrett2019probability}, we have $\sup_{x\in K}|p_{n}(x)-p(x)|\pto0$ as $n\to\infty$.
\end{proof}


\begin{lemma}\label{lem:point_unif_conv}
Consider a compact set $\cX$, and a class $\cF=\{f(x)\}$ of functions defined on $\cX$. Assume $\cF$ is uniformly Lipschitz continuous with respect to $x$, i.e., there exists $\ell_0$ so that for all $f\in\cF$,
\begin{equation*}
	\|f(x)-f(x')\|\leq \ell_0\|x-x'\|,\quad \forall x,x'\in\cX.
\end{equation*}
Let $f_n,n=1,2,\dots$ be a sequence of random functions from $\cF$ and $f_0\in\cF$ be a deterministic function. Suppose for all $x\in\cX$, we have $f_n(x)\pto f_0(x)$ as $n\to\infty$. Then we have $\sup_{x\in\cX}\|f_n(x)-f_0(x)\|\pto0$ as $n\to\infty$.
\end{lemma}

\begin{proof}
For simplicity, denote $f'_n(x)=f_n(x)-f_0(x)$. Then $\{f'_n(x)\}$ is uniformly Lipschitz continuous with constant $2\ell_0$.

Given any $\epsilon>0$ and $\delta>0$. Since $\cX$ is compact, it can be partitioned into a finite number $N_\delta$ of balls with radius no more than $\delta$, i.e., $B_j=\{x:\|x-x_j\|\leq\delta\}$ with $x_j$ being the center of the $j$th ball, $j=1,\dots,N_\delta$.  Then we have
\begin{align*}
	\bbP\left(\sup_{x\in\cX}\|f'_n(x)\|>\epsilon\right) &\leq \bbP\left(\max_j\sup_{x\in B_j}\left[\|f'_n(x)-f'_n(x_j)\|+\|f'_n(x_j)\|\right]>\epsilon\right)\\
	&\leq \bbP\left(\max_j\sup_{x\in B_j}\|f'_n(x)-f'_n(x_j)\|>\frac{\epsilon}{2}\right) + \bbP\left(\max_j\|f'_n(x_j)\|>\frac{\epsilon}{2}\right)\\
	&\leq \bbP\left(\sup_{\|x-x'\|<\delta}\|f'_n(x)-f'_n(x')\|>\frac{\epsilon}{2}\right) + \sum_{j=1}^{N_\delta}\bbP\left(\|f'_n(x_j)\|>\frac{\epsilon}{2}\right)\\
	&\leq \bbP\left(2\ell_0\delta>\frac{\epsilon}{2}\right) + \sum_{j=1}^{N_\delta}\bbP\left(\|f'_n(x_j)\|>\frac{\epsilon}{2}\right),
\end{align*}
where the third inequality follows from the union bound, and the last equality comes from the uniform Lipschitz continuity of $\{f'_n(x)\}$.
We let $n\to\infty$ to get rid of the second term by pointwise convergence, and further let $\delta\to0$ to get rid of the first term, which leads to the desired result.
\end{proof}



\begin{lemma}[Uniform continuous mapping theorem]\label{lem:ucmt}
	Let $X_n$, $X$ be random vectors defined on $\cX$. Let $f:\bbR^d\to\bbR^m$ be uniformly continuous and $T_\theta:\cX\to\bbR^d$ for $\theta\in\Theta$. Suppose $T_\theta(X_n)$ converges uniformly in probability to $T_\theta(X)$ over $\Theta$, i.e., as $n\to\infty$ we have  $\sup_{\theta\in\Theta}\|T_\theta(X_n)-T_\theta(X)\|\pto0$. Then $f(T_\theta(X_n))$ converges uniformly in probability to $f(T_\theta(X))$, i.e., $\sup_{\theta}\|f(T_\theta(X_n))-f(T_\theta(X))\|\pto0$.
\end{lemma}
\begin{proof}
Given any $\epsilon>0$. 
Because $f$ is uniformly continuous, there exists $\delta>0$ such that $\|f(x)-f(y)\|\leq\epsilon$ for all $\|x-y\|\leq\delta$.

We have
\begin{align}
\bbP\Big(\sup_{\theta\in\Theta}\|T_\theta(X_n)-T_\theta(X)\|\leq\delta\Big)&=\bbP\big(\forall\theta\in\Theta:\|T_\theta(X_n)-T_\theta(X)\|\leq\delta\big)\label{eq:ucmt1}\\
&\leq\bbP\big(\forall\theta\in\Theta:\|f(T_\theta(X_n))-f(T_\theta(X))\|\leq\epsilon\big)\nonumber\\
&=\bbP\Big(\sup_{\theta\in\Theta}\|f(T_\theta(X_n))-f(T_\theta(X))\|\leq\epsilon\Big)\label{eq:ucmt2}.
\end{align}
By the uniform convergence of $T_\theta(X_n)$, we know the left-hand side of (\ref{eq:ucmt1}) converges to 1.
Hence (\ref{eq:ucmt2}) goes to 1, which implies the desired result.
\end{proof}


\subsection{Proof of Theorem \ref{thm:grad_conv}}\label{app:pf_grad_conv}
\begin{proof}
The proof proceeds in three steps.

\medskip
\noindent
\textit{Step I} \ \ We first establish the consistency of $\hat{D}(x)$ to $D^*(x)$ as defined in (\ref{eq:d_conv}) below based on the generalization analysis of maximum likelihood estimation. Note that the analysis below (in this section) holds for all $\theta\in\Theta$ in a pointwise manner unless indicated otherwise, so for simplicity of notation, we omit the subscript $\theta$.

Following the probabilistic model in Section \ref{sec:age}, by the Bayes formula we have $\bbP(Y=1|x)= p_*(x)/((1+\lambda)p_0(x))$ and $\bbP(Y=0|x)=\lambda p_\theta(x)/((1+\lambda)p_0(x))$ which define the probability mass function $p_0(y|x)$, $y\in\{0,1\}$. Let the joint probability functions $p_D(x,y)=p_D(y|x)p_0(x)$ and $p_0(x,y)=p_0(y|x)p_0(x)$.
Let the class
\begin{equation*}
	\cG=\left\{g(x,y)=\frac{1}{2}\ln\frac{p_D(x,y)+p_0(x,y)}{2p_0(x,y)}:D\in\cD\right\}.
\end{equation*}
Note that each element of $\cG$ can be written as
\begin{equation*}
	g(x,y)=\frac{1}{2}\ln\frac{p_D(y|x)+p_0(y|x)}{2p_0(y|x)}.
\end{equation*}
%By the boundedness of $D^*$ in condition \ref{ass:D_bound}, we know the mass function $p_0(y|x)$ is bounded in a closed interval within $(0,1)$, so $g$ is uniformly bounded. 

Let $g_\infty=\sup_{g\in\cG}|g|$. From condition \ref{ass:envelope} we know that $\bbE_{p_0(x)}[\sup_{D\in\cD}|D(X)|]<\infty$. Note that when $|D|\leq1$, $|\ln(1/(1+e^{-D}))|\leq\ln(1+e)$; when $|D|>1$, $|\ln(1/(1+e^{-D}))|\leq |D|\ln(1+e)$. Both inequalities hold when we replace $D$ with $-D$. Thus
\begin{eqnarray*}
	&&\bbE_{p_0(x,y)}\left[\sup_{D\in\cD}|\ln(p_D(Y|X))|\right]\\
	&=&\frac{1}{1+\lambda}\bbE_{p_*(x)}\left[\sup_{D\in\cD}\left|\ln\left(1/(1+e^{-D(X)}\lambda)\right)\right|\right]+\frac{\lambda}{1+\lambda}\bbE_{p_\theta(x)}\left[\sup_{D\in\cD}\left|\ln\left(1/(1+e^{D(X)}/\lambda)\right)\right|\right]\\
		&=&\frac{1}{1+\lambda}\bbE_{p_*(x)}\left[\sup_{D\in\cD}\left|\ln\left(1/(1+e^{-D}\lambda)\mathbf{1}_{(|D-\ln\lambda|\leq1)}\right)+\ln\left(1/(1+e^{-D}\lambda)\mathbf{1}_{(|D-\ln\lambda|>1)}\right)\right|\right]\\
	&&+\frac{\lambda}{1+\lambda}\bbE_{p_\theta(x)}\left[\sup_{D\in\cD}\left|\ln\left(1/(1+e^{D}/\lambda)\mathbf{1}_{(|D-\ln\lambda|\leq1)}\right)+\ln\left(1/(1+e^{D}/\lambda)\mathbf{1}_{(|D-\ln\lambda|>1)}\right)\right|\right]\\
	&\leq &\ln(1+e)\cdot\left(1+\ln\lambda+\bbE_{p_0(x)}\left[\sup_{D\in\cD}|D(X)|\right]\right)<\infty.
\end{eqnarray*}
Hence we have $\bbE_{p_0(x,y)}[g_\infty(x,y)]<\infty$. 
Moreover for all $\delta>0$, the compactness of $\cD$ assumed in condition \ref{ass:d_compact} implies a finite bracketing covering number defined in Definition \ref{def:cover_num}, i.e., $N_{1,B}(\delta,\cD,\mu^*)<\infty$, where $\mu^*$ is the induced probability measure of density $p_0$. Then it follows from \cite[Theorem~4.3]{geer2000empirical} that  
\begin{equation}\label{eq:conv_in_h}
	H(p_{\hat{D}}(x,y),p_0(x,y))\to0
\end{equation}
almost surely as $n\to\infty$.

Consider any compact subset $K$ of $\cX$. We know from conditions \ref{ass:D_bound} and \ref{ass:D_cont} that for all $D\in\cD$, $D(x)$ is uniformly bounded and Lipschitz on $K$. Then $\cP=\{P_D(Y=1|x):D\in\cD\}$ is uniformly bounded and Lipschitz on $K$. Further since $p_0(x)$ is continuous and hence bounded and Lipschitz on $K$, we know $\{p_D(x,y)=p_0(x)p_D(y|x)\}$ is uniformly bounded and Lipschitz with respect to $x$.

Also from the boundedness of $D^*(x)$ on $K$, we know that $p_0(x)$ is bounded away from 0 on $K$. Then it follows from (\ref{eq:conv_in_h}) and Lemma \ref{lem:conv_density} that
\begin{equation*}
	\sup_{x\in K}|\hat{P}(Y=1|x)-\bbP(Y=1|x)|\pto0.
\end{equation*}
Then by continuous mapping theorem (Lemma \ref{lem:ucmt}) and noting that $l(p)=\ln(\lambda p/(1-p))$ is uniformly continuous on a closed interval within $(0,1)$, we have as $n\to\infty$
\begin{equation}\label{eq:d_conv}
	\sup_{x\in K}|\hat{D}(x)-D^*(x)|\pto0.
\end{equation}
This directly implies the pointwise convergence, i.e., for all $x\in\cX$, as $n\to\infty$, $|\hat{D}(x)-D^*(x)|\pto0$. 
Further from the smoothness in condition \ref{ass:D_smooth} and the compactness of $\Theta$, for all $x$, by applying Lemma \ref{lem:point_unif_conv} to function class $\{D(x)- D_{\theta}^*(x):D\in\cD\}$ of $\theta$, we have as $n\to\infty$
\begin{equation}\label{eq:d_conv_unif}
	\sup_{\theta\in\Theta}|\hat{D}(x)-D_\theta^*(x)|\pto0.
\end{equation}


\medskip\noindent
\textit{Step II} \ \  We then prove the consistency of the gradient $\nabla \hat{D}(x)$ to $\nabla D^*(x)$ as defined in (\ref{eq:d_grad_conv}).

Construct an arbitrary probability measure $\mu$ on $\cX$ that satisfies the following (e.g., any Gaussian measure):
\begin{itemize}\vspace{-0.1cm}
\setlength{\itemsep}{0pt}
%\setlength{\parskip}{0pt}
\item $\mu$ is absolutely continuous with respect to Lebesgue measure with a density $\rho$.
%\item \tbm{$\mu$ is tight, i.e., for any $\epsilon>0$, there is a compact subset $K_\epsilon$ of $\cX$ such that $\mu(K_\epsilon)>1-\epsilon$.}
%\item \tbm{$\nabla\ln\rho$ is uniformly bounded, i.e., there exists $B_1>0$ such that $\|\nabla\ln\rho(x)\|\leq B_1$ for all $x\in \cX$.}
\item $\rho$ vanishes at infinity rapidly enough, i.e., $\rho(x)=o(\|x\|^{-d})$. 
\item Log density $\ln\rho$ is continuously differentiable.
\end{itemize}%\vspace{-0.3cm}

Let $B_r=\{x\in\cX:\|x\|\leq r\}$ and $B_r^c=\cX\setminus B_r$ be the complement. Then by condition \ref{ass:D_bound}, there exists an upper bound $B>0$ so that for all $x\in B_r$ and $D\in\cD$, we have $|D(x)|\leq B$, $\|\nabla D(x)\|\leq B$, $|tr(\nabla^2 D(x))|\leq B$, and $\|\nabla\ln\rho(x)\|\leq B$.

We write 
\begin{equation}\label{eq:decom_ball}
	\int_{\cX} \|\nabla\hat{D}(x)-\nabla D^*(x)\|^2d\mu = \int_{B_r} \|\nabla\hat{D}(x)-\nabla D^*(x)\|^2d\mu + \int_{B_r^c} \|\nabla\hat{D}(x)-\nabla D^*(x)\|^2d\mu.
\end{equation}

We first deal with the first term in (\ref{eq:decom_ball}). 
For a function $u$ that is uniformly bounded on $\cX$, we have from integration by parts and Cauchy-Schwartz inequality that 
\begin{align*}
	\int\|\nabla u\|^2d\mu &= -\int u\ tr(\nabla^2u)d\mu-\int u\nabla u^\top \nabla\ln\rho d\mu\nonumber\\
	&\leq \sqrt{\int|u|^2d\mu\int [tr(\nabla^2u)]^2d\mu} + \sqrt{\int|u|^2d\mu\int(\nabla u^\top \nabla\ln\rho)^2d\mu}.\label{eq:ibp1}
\end{align*}

By noting the boundedness of any continuous functions on a compact ball, we have for all $\theta\in\Theta$ that
\begin{equation}\label{eq:in1}
	\int_{B_r} \|\nabla\hat{D}(x)-\nabla D^*(x)\|^2d\mu\leq (2B+\sqrt{2}B^2)\sqrt{\int_{B_r}|\hat{D}(x)-D^*(x)|^2d\mu}.
\end{equation}

By the uniform convergence in (\ref{eq:d_conv}) over compact ball $B_r$, we have for all $x\in B_r$, there exists a sequence $a_{n}=o_p(1)$ which is free of $x$ such that $|\hat{D}(x)-D(x)|^2\leq a_{n}$. Then we have
\begin{equation}\label{eq:in2}
	\int_{B_r}|\hat{D}(x)-D^*(x)|^2d\mu \leq \int_{B_r}a_{n}d\mu = a_{n}\mu(B_r)=o_p(1),
\end{equation}
by noting that $\mu$ is finite. 

We then handle the second term in (\ref{eq:decom_ball}). Let $\tilde{D}(x)=\sup_{D\in\cD}\|\nabla D(x)\|$. Note that
\begin{equation*}
\begin{split}
	\|\nabla\hat{D}(x)-\nabla D^*(x)\|&\leq\sup_{D\in\cD,D'\in\cD^*}\|\nabla D(x)-\nabla D'(x)\|\\
	&\leq \sup_{D\in\cD}\|\nabla D(x)\|+\sup_{D'\in\cD^*}\|\nabla D'(x)\|\\
	&\leq 2\tilde{D}(x).
\end{split}
\end{equation*}
From condition \ref{ass:envelope} we know $\bbE_\mu[\tilde{D}(X)]<\infty$. Also we have $\tilde{D}(X)\mathbf{1}_{X\in B_r^c}\to0$ as $r\to\infty$. Hence by the dominated convergence theorem we have 
\begin{equation}\label{eq:out}
	\int_{B_r^c} \|\nabla\hat{D}(x)-\nabla D^*(x)\|^2d\mu \leq 2\int_{B_r^c} \tilde{D}(x)d\mu\to0,
\end{equation}
as $r\to\infty$, which holds for all $n$ (the inequality holds uniformly for all $n$).

Combining (\ref{eq:decom_ball}-\ref{eq:out}) we have as $n\to\infty$
\begin{equation*}
	\int_{\cX} \|\nabla\hat{D}(x)-\nabla D^*(x)\|^2d\mu\pto0.
\end{equation*}
Recall the arbitrariness of $\mu$. For all $x\in\cX$, construct $\mu$ such that $\rho(x)>0$. 
Let $v(x)=\|\nabla\hat{D}(x)-\nabla D^*(x)\|^2\rho(x)$.
By the converse of the mean value theorem, if $x$ is not an extremum of $v$, then there exists a bounded subset $\cS(x)\subseteq\cX$ such that 
\begin{align*}
	\|\nabla\hat{D}(x)-\nabla D^*(x)\|^2\rho(x)&= \frac{1}{\nu(\cS(x))}\int_{\cS(x)}v(x')dx' \\
	&\leq \frac{1}{\nu(\cS(x))}\int_{\cX} v(x')dx'\pto0
\end{align*}
where $\nu$ denotes the Lebesgue measure. Since $\rho(x)>0$, this implies $\|\nabla\hat{D}(x)-\nabla D^*(x)\|\pto0$ for all non-extrema. By Lipschitz continuity of $v$ on any compact set, we have $\|\nabla\hat{D}(x)-\nabla D^*(x)\|\pto0$ for all extrema. 

Up to now we have shown that for all $\theta\in\Theta$ and $x\in\cX$, we have $\|\nabla\hat{D}(x)-\nabla D^*(x)\|\pto0$ as $n\to\infty$. 
Further from the smoothness in condition \ref{ass:D_smooth} and the compactness of $\Theta$, for all $x$, by applying Lemma \ref{lem:point_unif_conv} to function class $\{\nabla D(x)-\nabla D_{\theta}^*(x):D\in\cD\}$ of $\theta$, we have as $n\to\infty$
\begin{equation}\label{eq:d_grad_conv}
	\sup_{\theta\in\Theta}\|\nabla\hat{D}(x)-\nabla D^*(x)\|\pto0.
\end{equation}


\medskip
\noindent
\textit{Step III} \ \  Based on the convergence statements developed above, we proceed to show the consistency of the approximate gradient $h_{\hat{D}}(\theta)$ and complete the proof.

On one hand, from the tightness of $\Theta$ and $\cD$, dominated convergence in condition \ref{ass:emp_envelop}, and the uniform law of large numbers, we have as $n\to\infty$,
\begin{equation*}
	\sup_{\theta\in\Theta,D\in\cD}\|h_{D}(\theta)-\bbE_{p_z}[h_D'(Z;\theta)]\|\pto0,
\end{equation*}
which implies
\begin{equation*}
	\sup_{\theta\in\Theta}\|h_{\hat D}(\theta)-\bbE_{p_z}[h_{\hat D}'(Z;\theta)]\|\pto0.
\end{equation*}

On the other hand, we know from (\ref{eq:d_conv_unif}), (\ref{eq:d_grad_conv}), and the continuous mapping theorem (Lemma \ref{lem:ucmt}) that for any compact subset $K'$ of $\cZ$, as $n\to\infty$, we have
\begin{equation}\label{eq:h_unif}
	\sup_{\theta\in\Theta,z\in K'}\|h'_{\hat{D}}(z;\theta)-h'_{D^*}(z;\theta)\|\pto0.
\end{equation}
Let $B'_r=\{z\in\cZ:\|z\|\leq r\}$ and ${B'_r}^c=\cZ\setminus B_r$. 
Note that 
\begin{eqnarray}
	\sup_{\theta\in\Theta}\big\|\bbE[h_{\hat D}'(Z;\theta)]-\bbE[h_{D^*}'(Z;\theta)]\big\|&\leq& \bbE\left[\sup_{\theta\in\Theta}\|h_{\hat D}'(Z;\theta)-h_{D^*}'(Z;\theta)\|\right]\label{eq:h_conv_decom}\\
	&=&\bbE_{B'_r}\left[\sup_{\theta\in\Theta}\|h_{\hat D}'(Z;\theta)-h_{D^*}'(Z;\theta)\|\right]\label{eq:h_conv_in}\\
	&&+\bbE_{{B'_r}^c}\left[\sup_{\theta\in\Theta}\|h_{\hat D}'(Z;\theta)-h_{D^*}'(Z;\theta)\|\right].\label{eq:h_conv_out}
\end{eqnarray}
From (\ref{eq:h_unif}) we know (\ref{eq:h_conv_in}) vanishes in probability. Similar to the derivation of (\ref{eq:out}), by dominated convergence theorem and condition \ref{ass:emp_envelop}, we know (\ref{eq:h_conv_out}) vanishes in probability. Hence we know the left-hand side of (\ref{eq:h_conv_decom}) vanishes in probability. 

Note that $\nabla L(\theta)=\bbE_{Z} [h_{D^*}'(Z;\theta)]$. By the triangle inequality, we have 
\begin{equation*}
	\sup_{\theta\in\Theta}\|h_{\hat D}(\theta)-\nabla L(\theta)\|\leq\sup_{\theta\in\Theta}\|h_{\hat D}(\theta)-\bbE_{Z}[h_{\hat D}'(Z;\theta)]\| + \sup_{\theta\in\Theta}\|\bbE_{Z}[h_{\hat D}'(Z;\theta)]-\nabla L(\theta)\|.
\end{equation*}

Therefore, as $n\to\infty$ we have
\begin{equation*}
	\sup_{\theta\in\Theta}\|h_{\hat D}(\theta)-\nabla L(\theta)\|\pto0,
\end{equation*}
which completes the proof.	
\end{proof}


\subsection{Proof of Theorem \ref{thm:cons}}\label{app:pf_cons}

\begin{proof}
We recall the approximate gradient descent step in Algorithm \ref{alg:age}
\begin{equation*}
	\theta_t = \theta_{t-1} - \eta h_{\hat D_t}(\theta_{t-1}),
\end{equation*}
where $\eta>0$ is the learning rate.
Suppose $L(\theta)$ is $\ell_0$-smooth. Then we have
\begin{equation*}
	L(\theta_t) \leq L(\theta_{t-1}) - \eta h_{\hat D_t}(\theta_{t-1})^\top\nabla L(\theta_{t-1}) + \frac{\eta^2\ell_0}{2}h_{\hat D_t}(\theta_{t-1})^\top h_{\hat D}(\theta_{t-1}).
\end{equation*}

Let $\hat\delta(\theta)=\nabla L(\theta)-h_{\hat{D}}(\theta)$. By Theorem \ref{thm:grad_conv}, as $n\to\infty$, $\hat\delta=\sup_{\theta}\|\hat\delta(\theta)\|\pto0$. Then we have
\begin{align*}
	-\eta h_{\hat D_t}(\theta_{t-1})^\top\nabla L(\theta_{t-1})&=-\eta h_{\hat D_t}(\theta_{t-1})^\top\left(h_{\hat D_t}(\theta_{t-1})+\hat\delta(\theta_{t-1})\right)\\
	&\leq \eta \left(-\|h_{\hat D_t}(\theta_{t-1})\|^2 +(\|h_{\hat D_t}(\theta_{t-1})\|^2+\|\hat\delta\|^2)/2\right)\\
	&=-\frac{\eta}{2}\left(\|h_{\hat D_t}(\theta_{t-1})\|^2-\hat\delta^2\right)\\
	&\leq -\frac{\eta}{4}\|h_{\hat D_t}(\theta_{t-1})\|^2,
\end{align*}
under the case where $\|h_{\hat D_t}(\theta_{t-1})\|^2\geq 2\hat\delta^2$. We note that
\begin{align*}
	L(\theta_t) &\leq L(\theta_{t-1}) - \frac{\eta}{4}\|h_{\hat D_t}(\theta_{t-1})\|^2 + \frac{\eta^2\ell_0}{2}\|h_{\hat D_t}(\theta_{t-1})\|^2\\
	&\leq L(\theta_{t-1}) - \frac{\eta}{8}\|h_{\hat D_t}(\theta_{t-1})\|^2,
\end{align*}
when $\eta<1/4\ell_0$, which can be satisfied with a sufficiently small learning rate.

By summing over $t=1,\dots,T$, we have  
\begin{equation*}
	L(\theta_T) \leq L(\theta_0) - 0.125 \eta \sum_{t=1}^T \|h_{\hat D_t}(\theta_{t-1})\|^2.
\end{equation*}
Note that $L(\theta)$ is lower bounded by 0. Then we have $\sum_{t=1}^T \|h_{\hat D_t}(\theta_{t-1})\|^2 = O(1)$. Thus there exists $t$ in $\{0,\dots,T\}$ such that $\|h_{\hat D_t}(\theta_{t-1})\|^2 = O(1/T)=O(1/n)$, since we set $T=O(n)$. 

Otherwise there exists $t$ such that $\|h_{\hat D_t}(\theta_{t-1})\|<\sqrt{2}\hat\delta=o_p(1)$.% and hence we have $\|h_{\hat D}(\theta_{t-1})\|\to0$.

Therefore, by combining the two cases, we have 
\begin{equation*}
	\hat\theta\in\{\theta:\|h_{\hat D}(\theta)\|=o_p(1)\}.
\end{equation*} 

Furthermore, by the strong convexity of $L(\theta)$, we have $\nabla L(\theta^*)=0$ and for arbitrary $\epsilon>0$,
\begin{equation*}
	\inf_{\theta\in\Theta\setminus B(\theta^*,\epsilon)}\|\nabla L(\theta)\|>0.
\end{equation*}
where $B(\theta^*,\epsilon)=\{\theta\in\Theta:\|\theta-\theta^*\|<\epsilon\}$ is an open ball. 
By the uniform convergence (\ref{eq:unif_grad}) from Theorem \ref{thm:grad_conv}, we have $\|h_{\hat{D}}(\theta^*)\|\pto\|\nabla L(\theta^*)\|=0$ and 
\begin{equation*}
	\inf_{\theta\in\Theta\setminus B(\theta^*,\epsilon)}\|h_{\hat{D}}(\theta)\|\pto\inf_{\theta\in\Theta\setminus B(\theta^*,\epsilon)}\|\nabla L(\theta)\|>0.
\end{equation*}
%
Hence we have $\bbP(\hat\theta\in B(\theta^*,\epsilon))\to1$. 
By the arbitrariness of $\epsilon$, we have $\hat\theta\pto\theta^*$ as $n\to\infty$.
\end{proof}


\subsection{Proof of Theorem \ref{thm:d_par_cons}}\label{app:pf_d_par_cons}
\begin{proof}
Given arbitrary $\epsilon>0$. Let $B(\psi^*,\epsilon)=\{\psi\in\Psi: \|\psi-\psi^*\|<\epsilon\}$. We have 
$$
\min_{\psi\in\Psi \setminus B(\psi^*,\epsilon)} L_d(\psi)>L_d(\psi^*).
$$
By the weak law of large numbers, we have $\hat{L}_d(\psi^*)\pto L_d(\psi^*)$ as $n\to\infty$. By the uniform law of large numbers, we have 
$$
\max_{\psi\in\Psi \setminus B(\psi^*,\epsilon)}|\hat{L}_d(\psi)- L_d(\psi)|\pto0,
$$
as $n\to\infty$, which implies 
$$
\min_{\psi\in\Psi \setminus B(\psi^*,\epsilon)}\hat{L}_d(\psi)\pto\min_{\psi\in\Psi \setminus B(\psi^*,\epsilon)}{L}_d(\psi)>L_d(\psi^*),
$$
and then $\bbP(\hat{\psi}\in B(\psi^*,\epsilon))\to1$ as $n\to\infty$. Since $\epsilon$ is arbitrary, we have $\hat{\psi}\pto \psi^*$ as $n\to\infty$.
\end{proof}


\subsection{Proof of Theorem \ref{thm:d_asy_norm}}\label{app:pf_d_eff}

\begin{proof}%[Proof of Theorem \ref{thm:d_asy_norm}]
By consistency and Taylor expansion, we have 
\begin{equation*}
	\nabla_\psi \hat{L}_d(\hat\psi)-\nabla_\psi \hat{L}_d(\psi^*) = \nabla^2_\psi \hat{L}_d(\psi^*)(\hat\psi-\psi^*)+O_p(\|\hat\psi-\psi^*\|^2),
\end{equation*}
where we note $\nabla_\psi \hat{L}_d(\hat\psi)=0$.
Then
\begin{equation*}
	\sqrt{n}\left(\hat{\psi}-\psi^*\right)=-\left[\nabla^2_\psi \hat{L}_d(\psi^*)\right]^{-1}\left[\frac{1}{\sqrt{n}}\sum_{i=1}^n\nabla_{\psi}l_1(x_i;\psi^*)+\frac{1}{\sqrt{\lambda m}}\sum_{i=1}^m\nabla_{\psi}l_2(z_i;\psi^*)\right]+O_p\left(\frac{\|\sqrt{n}(\hat\psi-\psi^*)\|^2}{\sqrt{n}}\right).
\end{equation*}
By the weak law of large numbers, we have $$\nabla^2_\psi \hat{L}_d(\psi^*)\pto\nabla^2_\psi L_d(\psi^*)=H_d\succ0$$ by condition \ref{ass:pos_hess}. 

By the central limit theorem and independence, we have as $n\to\infty$,
\begin{equation*}
	\frac{1}{\sqrt{n}}\sum_{i=1}^n\nabla_{\psi}l_1(x_i;\psi^*)+\frac{1}{\sqrt{\lambda m}}\sum_{i=1}^m\nabla_{\psi}l_2(G_\theta(z_i);\psi^*)\dto\cN(0,V_d)
\end{equation*}
where $V_d=V_1+V_2/\lambda$, $V_1=\mathrm{Var}(\nabla_\psi l_1(X;\psi^*))$, and $V_2=\mathrm{Var}(\nabla_\psi l_2(G_\theta(Z);\psi^*))$. Then we have
\begin{align*}
	V_d&=\bbE_{p_*}[\nabla_{\psi}l_1(X;\psi^*)\nabla_{\psi}l_1(X;\psi^*)^\top]+\bbE_{p_\theta}[\nabla_{\psi}l_2(X;\psi^*)\nabla_{\psi}l_2(X;\psi^*)^\top]/\lambda\\
	&\ \ -(1+1/\lambda)\bbE_{p_*}[\nabla_{\psi}l_1(X;\psi^*)]\bbE_{p_*}[\nabla_{\psi}l_1(X;\psi^*)]^\top.
\end{align*}

By the Slutsky's theorem, we have as $n\to\infty$,
\begin{equation*}
\sqrt{n}\left(\hat{\psi}-\psi^*\right)\dto\cN(0,\Sigma_d),
\end{equation*}
where $\Sigma_d=H_d^{-1}V_dH_d^{-1}$.
\end{proof}


\subsection{Proof of Theorem \ref{thm:f_d_asy_norm}}\label{app:pf_f_d_eff}
\begin{proof} 
	We can show the asymptotic normality of $\hat\psi_f$ by the arguments similar to those in the proof of Theorem \ref{thm:d_asy_norm}, where $l_i$ is replaced by $l^f_i$ for $i=1,2$.
\end{proof}


\subsection{Proof of Lemma \ref{lem:g_cons}}\label{app:pf_g_cons}
\begin{proof}
Given arbitrary $\epsilon>0$. Let $B(\theta^*,\epsilon)=\{\theta\in\Theta:\|\theta-\theta^*\|<\epsilon\}$. By definition we have 
\begin{equation*}
	\min_{\theta\in\Theta\setminus B(\theta^*,\epsilon)}L(\theta)>L(\theta^*).
\end{equation*}
Note that $\hat L'(\theta):=\hat L(\theta)+\hat\epsilon(\theta^*)^\top\theta$ where
\begin{equation*}
	\hat\epsilon(\theta^*)=h_{\hat{D}}(\theta^*)-\nabla{L}(\theta^*)+\nabla{L}(\theta^*)-\nabla\hat{L}(\theta^*).
\end{equation*}
We know from Theorem \ref{thm:grad_conv} that as $n\to\infty$, $\|h_{\hat{D}}(\theta^*)-\nabla{L}(\theta^*)\|\pto0$, and from the weak law of large numbers that $\|\nabla{L}(\theta^*)-\nabla\hat{L}(\theta^*)\|\pto0$. Hence $\|\hat\epsilon(\theta^*)\|\pto0$ as $n\to\infty$. Also note $\|\theta\|$ is bounded.
Further by the uniform law of large numbers, we have
\begin{equation*}
	\sup_{\theta\in\Theta}|\hat L'(\theta)-L(\theta)|=\sup_{\theta\in\Theta}|\hat L(\theta)-L(\theta)|+o_p(1)\pto0,
\end{equation*}
as $n\to\infty$, which implies $\hat L'(\theta^*)\pto L(\theta^*)$ and 
\begin{equation*}
	\min_{\theta\in\Theta\setminus B(\theta^*,\epsilon)}\hat L'(\theta) \pto \min_{\theta\in\Theta\setminus B(\theta^*,\epsilon)}L(\theta)>L(\theta^*).
\end{equation*}
Then $\bbP(\theta'\in B(\theta^*,\epsilon))\pto1$ as $m,n\to\infty$. Since $\epsilon$ is arbitrary, we have $\theta'\pto\theta^*$ as $n\to\infty$. The consistency of $\tilde\theta$ can be obtained similarly.
\end{proof}


\subsection{Proof of Theorem \ref{thm:g_rate}}\label{app:pf_g_rate}

\begin{proof}

After establishing the consistency of $\tilde\theta$, $\theta'$ and $\hat\theta$, we have the following basic expansions which will be used later.
\begin{equation}\label{eq:ttheta}
\underbrace{\nabla \hat L(\tilde\theta)}_{=0}-\nabla\hat L(\theta^*)=\nabla^2\hat{L}(\theta^*)(\tilde\theta-\theta^*)+O_p(\|\tilde\theta-\theta^*\|^2),
\end{equation}
\begin{equation}\label{eq:theta'}
{\underbrace{\nabla \hat L'(\theta')}_{=0}}-\underbrace{\nabla\hat L'(\theta^*)}_{=\nabla\hat L(\theta^*)+\hat\epsilon(\theta^*)}=\underbrace{\nabla^2\hat{L}'(\theta^*)}_{=\nabla^2\hat{L}(\theta^*)}(\theta'-\theta^*)+O_p(\|\theta'-\theta^*\|^2),
\end{equation}
\begin{equation}\label{eq:htheta}
\nabla \hat L'(\hat\theta)-\nabla\hat L'(\theta^*)=\nabla^2\hat{L}'(\theta^*)(\hat\theta-\theta^*)+O_p(\|\hat\theta-\theta^*\|^2).
\end{equation}

\medskip\noindent
\textit{Step I \ \ Convergence rate of $\tilde\theta-\theta^*$}
%\medskip

By manipulating (\ref{eq:ttheta}), we have 
\begin{equation}\label{eq:o1}
\tilde\theta-\theta^* = \gamma_n+O_p(1/n),
\end{equation}
where 
\begin{equation*}
	\gamma_n=-\left[\nabla^2\hat{L}(\theta^*)\right]^{-1}\nabla\hat L(\theta^*)
\end{equation*}
satisfies $\sqrt{n}\gamma_n=\sqrt{m/\lambda}\gamma_n\dto \cN(0,H_g^{-1}\Sigma_g H_g^{-1}/\lambda)$ as $n\to\infty$ with  $H_g=\bbE[\nabla^2l_g(\theta^*)]$ and $\Sigma_g=\bbE[\nabla l_g(\theta^*)\nabla l_g(\theta^*)^\top]$.

\bigskip\noindent
\textit{Step II \ \ Convergence rate of $\theta'-\tilde\theta$}

Taking (\ref{eq:ttheta}) $-$ (\ref{eq:theta'}) gives 
\begin{equation}\label{eq:bias}
\hat\epsilon(\theta^*)=\nabla^2\hat{L}(\theta^*)(\tilde\theta-\theta')+O_p(\|\tilde\theta-\theta^*\|^2+\|\theta'-\theta^*\|^2).
\end{equation}

Write $\hat\epsilon(\theta)=\hat\epsilon_1(\theta)+\hat\epsilon_2(\theta)$ where $\hat\epsilon_1(\theta)=h_{\hat{D}}(\theta)-h_{D^*}(\theta)$ and $\hat\epsilon_2(\theta)=h_{D^*}(\theta)-\nabla\hat{L}(\theta)$.
We have
\begin{equation*}
	\hat\epsilon_{1}(\theta)=-\frac{1}{m}\sum_{i=1}^m \left[\nabla_\theta G_\theta(z_i)^\top \left(\hat{s}_g(G_\theta(z_i))\nabla_x \hat{D}(G_\theta(z_i))-s^*_g(G_\theta(z_i))\nabla_x D^*(G_\theta(z_i))\right) \right],
\end{equation*}
where $\hat{s}_g(x)=s_g(x;\hat{D})$.

For any $x,x'\in\mathcal{X}$, we have
\begin{align*}
\hat{s}_g(x')D_{\hat{\psi}}(x)-s^*_g(x')D_{\psi^*}(x)&=\nabla_{\psi} [s^*_g(x')D_{\psi^*}(x)]^\top(\hat\psi-\psi^*)+O_p(1/n)\\
&=\nabla_{\psi} [s^*_g(x')D_{\psi^*}(x)]^\top\xi'_n+O_p(1/n),
\end{align*}
where 
\begin{equation*}
	\xi'_n=-\left[\nabla^2_\psi \hat{L}_d(\psi^*)\right]^{-1}\left[\frac{1}{n}\sum_{i=1}^n\nabla_{\psi}l_1(x_i;\psi^*)+\frac{1}{m}\sum_{i=1}^m\nabla_{\psi}l_2(G_{\theta^*}(z_i);\psi^*)\right]
\end{equation*}
satisfies $\sqrt{n}\xi'_n\dto\cN(0,\Sigma_d)$ from Theorem \ref{thm:d_asy_norm}.

Then we have 
\begin{eqnarray}
%\hspace{-0.3in}
&&\hat{s}_g(x)\nabla_x \hat{D}(x)-s^*_g(x)\nabla_x D^*(x)\nonumber\\
&=&\hat{s}_g(x)\lim_{\|\delta\|\to0}\frac{\hat{D}(x+\delta)-\hat{D}(x)}{\|\delta\|}-s^*_g(x)\lim_{\|\delta\|\to0}\frac{{D^*}(x+\delta)-{D^*}(x)}{\|\delta\|}\nonumber\\
&=&\lim_{\|\delta\|\to0}\frac{\hat{s}_g(x)\hat{D}(x+\delta)-s^*_g(x){D^*}(x+\delta)-\left(\hat{s}_g(x)\hat{D}(x)-s^*_g(x){D^*}(x)\right)}{\|\delta\|}\nonumber\\
&=&\lim_{\|\delta\|\to0}\frac{\left(\nabla_\psi [s^*_g(x)D^*(x+\delta)]-\nabla_\psi [s^*_g(x)D^*(x)]\right)^\top}{\|\delta\|} \xi'_n+O_p(1/n) \nonumber\\
&=&\tilde\Sigma_g(x)\xi'_n+O_p(1/n),\label{eq:d_grad_expand}
\end{eqnarray}
where $\tilde\Sigma_g(x)=\nabla_\psi [s_g(x;D_\psi)\nabla_x D_\psi(x)]|_{\psi^*}$.


By (\ref{eq:d_grad_expand}), we have
\begin{equation}\label{eq:eps1_rate}
\begin{split}
	\hat\epsilon_{1}(\theta) &=-\frac{1}{m}\sum_{i=1}^m\left[\nabla_\theta G_\theta(z_i)^\top \left(\tilde\Sigma_g(G(z_i))\xi'_n+O_p(1/n)\right)  \right] \\
&= -\frac{1}{m}\sum_{i=1}^m\left[\nabla_\theta G_\theta(z_i)^\top\tilde\Sigma_g(G(z_i))\right]\xi'_n+O_p(1/n)\\
&= C_\theta {\xi'_n}+O_p(1/n)\\
&= \Sigma'(\theta){\xi_{n}^*}+O_p(1/n)
\end{split}
\end{equation}
where the second and third equalities follow from the central limit theorem, $$C_\theta=-\bbE[\nabla_\theta G_\theta(Z)^\top\tilde\Sigma_g(G(Z))]=\nabla_\psi\bbE[-s_g(G(Z);D_\psi)\nabla_\theta G_\theta(Z)^\top\nabla_x D_\psi(G(Z))]|_{\psi^*}=\nabla_\psi\bbE[h'_{D_{\psi^*}}(Z;\theta)]$$ (of $d_\theta\times d_\psi$), $\Sigma'(\theta)=C_\theta\Sigma_{d}^{1/2}$, and $\xi_{n}^*=\Sigma_d^{-1/2}\xi'_n$. %, and to obtain the last equality \textcolor{red}{we suppose the neighborhood $N(\theta^*)$ satisfies $\sup_{\theta\in N(\theta^*)}\|\Sigma_1(\theta)-\Sigma^1_{\theta^*}\|=O(1/\sqrt{n})$.}
% \tbm{some regularity conditions are needed to apply CLT, check!}

%By combining (\ref{eq:eps_theta}) and (\ref{eq:eps_phi}), we have
%\begin{equation}\label{eq:eps1_rate}
%	\hat\epsilon_1(\theta)={\Sigma'_{\theta}}{\xi_n^*}+O_p(1/n+1/m),
%\end{equation}
%where $C_{\theta}=(C_1(\theta)^\top,C_2(\phi)^\top)^\top=\nabla_\psi\bbE[h'_{D_\psi}(x,\epsilon,\epsilon';\theta)]|_{\psi^*(\theta^*)}$ and $\Sigma'_{\theta}=C_{\theta}\Sigma_{\theta}^{1/2}$.


Recall that 
\begin{equation*}
	\nabla L(\theta)=\bbE[\nabla l_g(Z;\theta)]=\bbE[h'(Z;\theta)],
\end{equation*}
\begin{equation*}
	\nabla\hat{L}(\theta)=\frac{1}{m}\sum_{i=1}^m\nabla l_g(z_i;\theta),\ h_{D^*}(\theta)=\frac{1}{m}\sum_{i=1}^m h'(z_i;\theta).
\end{equation*}
By the central limit theorem, we have as $n\to\infty$
\begin{equation}\label{eq:eps2_rate}
	\sqrt{n}\hat\epsilon_2(\theta)=\sqrt{\frac{m}{\lambda}}\hat\epsilon_2(\theta)\dto\cN(0,\Sigma_\tau(\theta)/\lambda),
\end{equation}
where $\Sigma_\tau(\theta)=\bbE[\tau\tau^\top]$ with $\tau=h'(x;\theta)-\nabla l_g(x;\theta)$.

Hence, for all fixed $\theta\in N(\theta^*)$, we have $\hat\epsilon(\theta)=O_p(1/\sqrt{n})$. 

(\ref{eq:eps1_rate}) and (\ref{eq:eps2_rate}), together with (\ref{eq:bias}), lead to 
\begin{equation}\label{eq:o2}
\theta'-\tilde\theta=\xi_n+\tau_n+O_p(1/n),
\end{equation}
where the first leading term 
\begin{equation*}
	\xi_n=-\left[\nabla^2\hat{L}(\theta^*)\right]^{-1}\Sigma'(\theta^*)\xi_n^*
\end{equation*}
satisfies $\sqrt{n}\xi_n\dto\cN(0,H_g^{-1}C\Sigma_{d,\theta^*} C^\top H_g^{-1})$ as $n\to\infty$, where $C=C_{\theta^*}$ and $\Sigma_{d,\theta^*}$ is the asymptotic variance of discriminator estimator $\hat\psi$ at the optimal generator $\theta^*$, and the second leading term
\begin{equation*}
	\tau_n=-\left[\nabla^2\hat{L}(\theta^*)\right]^{-1}\hat\epsilon_2(\theta^*)
\end{equation*}
satisfies $\sqrt{n}\tau_n\dto\cN(0,H_g^{-1}\Sigma_\tau H_g^{-1}/\lambda)$ as $n\to\infty$ with $\Sigma_\tau=\Sigma_\tau(\theta^*)$.


%\medskip
%--- rough rate ---

\bigskip\noindent
\textit{Step III \ \ $\sqrt{n}$-rate of convergence of $\hat\theta-\theta^*$}

%We then show that $\hat\theta-\theta'=O_p(1/\sqrt{n})$. 

Note that $\nabla \hat L'(\theta)=\nabla \hat L(\theta)+\epsilon(\theta^*)$ and the gradient used in Algorithm \ref{alg:age} is $h_{\hat D}(\theta)$. %We know from standard CLT that $\nabla \hat L(\theta)-h_{D^*}(\theta)=O_p(1/\sqrt{m})$. 
Let $\hat\delta'(\theta)=h_{\hat{D}}(\theta)-\nabla\hat L'(\theta)$ and $\hat\delta'=\sup_{\theta\in N(\theta^*)}\|\hat\delta'(\theta)\|$. Then from (\ref{eq:eps1_rate}) and (\ref{eq:eps2_rate}), we have for all $\theta\in N(\theta^*)$,
\begin{equation}\label{eq:grad_diff_decom}
\begin{split}
	\hat\delta'(\theta)&=\big[h_{D^*}(\theta)+h_{\hat{D}}(\theta)-h_{D^*}(\theta)\big]-\big[\nabla \hat L(\theta)+\epsilon_1(\theta^*)+\epsilon_2(\theta^*)\big]\\
	&=\hat\epsilon_1(\theta)-\hat\epsilon_1(\theta^*)+\hat\epsilon_2(\theta)-\hat\epsilon_2(\theta^*)=O_p(1/\sqrt{n})
\end{split}
\end{equation}
Since $N(\theta^*)$ is bounded, we have $\hat\delta'=O_p(1/\sqrt{n})$.

Suppose $\hat L'(\theta)$ is $\ell_0$-smooth. Then we have
\begin{equation*}
	\hat L'(\theta_t) \leq \hat L'(\theta_{t-1}) - \eta h_{\hat D_t}(\theta_{t-1})^\top\nabla \hat L'(\theta_{t-1}) + \frac{\eta^2\ell_0}{2}\|h_{\hat D_t}(\theta_{t-1})\|^2.
\end{equation*}
Under the case where $\|\nabla\hat L'(\theta_{t-1})\|^2\geq 2\hat\delta'^2$, we have
\begin{align*}
	- \eta h_{\hat D_t}(\theta_{t-1})^\top\nabla \hat L'(\theta_{t-1}) &= - \eta \left(\hat\delta'(\theta_{t-1})+\nabla\hat L'(\theta_{t-1})\right)^\top \nabla\hat L'(\theta_{t-1})\\
	&\leq \eta \left(-\|\nabla\hat L'(\theta_{t-1})\|^2 + (\|\nabla\hat L'(\theta_{t-1})\|^2+\hat\delta'^2)/2\right)\\
	&=-\frac{\eta}{2}\left(\|\nabla\hat L'(\theta_{t-1})\|^2-\hat\delta'^2\right)\\
	&\leq -\frac{\eta}{4}\|\nabla\hat L'(\theta_{t-1})\|^2,
\end{align*}
and
\begin{align*}
	\|h_{\hat D_t}(\theta_{t-1})\|^2 = \|\hat\delta'(\theta_{t-1})+\nabla\hat L'(\theta_{t-1})\|^2 \leq 2\big(\hat\delta'^2+\|\nabla\hat L'(\theta_{t-1})\|^2\big) \leq 3\|\nabla\hat L'(\theta_{t-1})\|^2.
\end{align*}
Then we have
\begin{align*}
	\hat L'(\theta_t) &\leq \hat L'(\theta_{t-1}) - \frac{\eta}{4}\|\nabla\hat L'(\theta_{t-1})\|^2 + \frac{3\eta^2\ell_0}{2}\|\nabla\hat L'(\theta_{t-1})\|^2\\
	&\leq \hat L'(\theta_{t-1}) - \frac{\eta}{8}\|\nabla\hat L'(\theta_{t-1})\|^2,
\end{align*}
when $\eta<1/12\ell_0$, which can be satisfied with a sufficiently small learning rate.

By summing over $t=1,\dots,T$, we have  
\begin{equation*}
	\hat L'(\theta_T) \leq \hat L'(\theta_0) - 0.125 \eta \sum_{t=1}^T \|\nabla\hat L'(\theta_{t-1})\|^2.
\end{equation*}
Note that $\hat L'(\theta)$ is lower bounded. Then we have $\sum_{t=1}^T \|\nabla\hat L'(\theta_{t-1})\|^2 = O_p(1)$. Thus there exists $t$ in $\{0,\dots,T\}$ such that $\|\nabla\hat L'(\theta_{t-1})\|^2 = O_p(1/T)=O_p(1/n)$, since we have $T=O(n)$.

Otherwise there exists $t$ such that $\|\nabla\hat L'(\theta_{t-1})\|<\sqrt{2}\hat\delta'$. 

Therefore we have $\|\nabla \hat L'(\hat\theta)\|=O_p(1/\sqrt{n})$.

Taking (\ref{eq:htheta}) $-$ (\ref{eq:theta'}) gives
\begin{equation}\label{eq:htheta-theta'}
	\nabla\hat{L}'(\hat\theta)=\nabla^2\hat{L}'(\theta^*)(\hat\theta-\theta')+O_p(\|\theta'-\theta^*\|^2+\|\hat\theta-\theta'\|^2),
\end{equation}
which further implies $\|\hat\theta-\theta'\|=O_p(1/\sqrt{n}).$
This, together with (\ref{eq:o1}) and (\ref{eq:o2}), implies
\begin{equation}\label{eq:rough_rate}
	\|\hat\theta-\theta^*\|=O_p(1/\sqrt{n}).
\end{equation}

%\medskip
%--- Specific rate ---

\bigskip\noindent
\textit{Step IV \ \ Convergence rate of $\hat\theta-\theta'$}

Based on (\ref{eq:rough_rate}), we suppose the neighborhood $N(\theta^*)$ satisfies $\sup_{\theta\in N(\theta^*)}\|\theta-\theta^*\|=O_p(1/\sqrt{n})$. On closed set $N(\theta^*)$, continuous function $\Sigma'(\theta)$ is Lipschitz continuous with respect to $\theta$ with Lipschitz constant $\ell_1$. Hence we have for all $\theta\in N(\theta^*)$
\begin{equation*}
	\|\Sigma'(\theta)-\Sigma'(\theta^*)\|\leq \ell_1 \|\theta-\theta^*\| = O_p(1/\sqrt{n}),
\end{equation*}
%\begin{equation*}
%	\|\hat\epsilon(\theta)-\hat\epsilon(\theta^*)\|\leq \ell_1 \|\theta-\theta^*\|\leq = O_p(1/\sqrt{m}+1/\sqrt{n})
%\end{equation*}
which is a uniform rate free of $\theta$. Then, by recalling (\ref{eq:eps1_rate}) and noting that $\xi^*_n=O_p(1/\sqrt{n})$, we further have
\begin{equation*}
	\hat\epsilon_1(\theta)={\Sigma'_{\theta^*}}\xi^*_n+O_p(1/n),
\end{equation*}
where the leading term is free of $\theta$, and the higher order term depends on $\theta$. 

Thus, we have for all $\theta\in N(\theta^*)$,
\begin{equation}\label{eq:grad_diff1}
	\hat\epsilon_1(\theta)-\hat\epsilon_1(\theta^*)=O_p(1/n).
\end{equation}



Similarly, on closed set $N(\theta^*)$, continuous function $\Sigma^{1/2}_\tau(\theta)$ is Lipschitz continuous with respect to $\theta$ with Lipschitz constant $\ell_2$. Hence we have for all $\theta\in N(\theta^*)$,
\begin{equation*}
	\|\Sigma^{1/2}_\tau(\theta)-\Sigma^{1/2}_\tau(\theta^*)\|\leq \ell_2 \|\theta-\theta^*\|\leq = O_p(1/\sqrt{n}).
\end{equation*}
Let $\hat\epsilon_2(\theta)=\Sigma^{1/2}_\tau(\theta)\tau^*_n$. Recalling (\ref{eq:eps2_rate}), then $\sqrt{n}\tau^*_n\dto\cN(0,I/\lambda)$ and $\tau^*_n=O_p(1/\sqrt{n})$ free of $\theta$. 
Thus, we have for all $\theta\in N(\theta^*)$
\begin{equation*}
	\hat\epsilon_2(\theta)=\Sigma^{1/2}_\tau(\theta)\tau^*_n=\Sigma^{1/2}_\tau(\theta^*)\tau^*_n+O_p(1/n),
\end{equation*}
where the leading term is also free of $\theta$. 

Thus, we have for all $\theta\in N(\theta^*)$,
\begin{equation}\label{eq:grad_diff2}
	\hat\epsilon_2(\theta)-\hat\epsilon_2(\theta^*)=O_p(1/n).
\end{equation}


By combining (\ref{eq:grad_diff1}) and (\ref{eq:grad_diff2}) and recalling the decomposition in (\ref{eq:grad_diff_decom}), we have for all $\theta\in N(\theta^*)$
\begin{equation*}
	\hat\delta'(\theta)=\hat\epsilon_1(\theta)-\hat\epsilon_1(\theta^*)+\hat\epsilon_2(\theta)-\hat\epsilon_2(\theta^*)=O_p(1/n),
\end{equation*}
and then $\hat\delta'=O_p(1/n)$. Then by analyzing the algorithm similarly as above, we eventually obtain $\|\nabla \hat L'(\hat\theta)\|=O_p(1/n)$.

Then by recalling (\ref{eq:htheta-theta'}), we have 
\begin{equation}\label{eq:o3}
	\|\hat\theta-\theta'\|=O_p(1/n),
\end{equation}
which is a higher order term. Therefore, the proof is completed.
\end{proof}



\subsection{Proof of Theorem \ref{thm:asy_normal}}\label{app:pf_asy_normal}
\begin{proof}
This proof is based on that of Theorem \ref{thm:g_rate}. By combining (\ref{eq:o1}) and (\ref{eq:o2}), we have
\begin{equation}\label{eq:o12}
	\theta'-\theta^*=\gamma_n+\tau_n+\xi_n+O_p(1/n)=\zeta_n+\xi_n+O_p(1/n),
\end{equation}
where 
\begin{equation*}
	\zeta_n=\gamma_n+\tau_n=\left[\nabla^2\hat{L}(\theta^*)\right]^{-1}\left[-\nabla\hat{L}(\theta^*)-h_{D^*}(\theta^*)+\nabla\hat{L}(\theta^*)\right]=-\left[\nabla^2\hat{L}(\theta^*)\right]^{-1}h_{D^*}(\theta^*)
\end{equation*}
satisfies $\sqrt{n}\zeta_n\dto\cN(0,H_g^{-1}\Sigma_h H_g^{-1}/\lambda)$ with $\Sigma_h=\bbE[h'(Z;\theta^*)h'(Z;\theta^*)^\top]$.
(\ref{eq:o12}), together with (\ref{eq:o3}), leads to
\begin{equation}\label{eq:hattheta}
	\hat\theta-\theta^*= \zeta_n+\xi_n+O_p(1/n).
\end{equation}
By the definition of $\zeta_n$ and $\xi_n$ and the central limit theorem, we have the asymptotic normality 
\begin{equation*}
	\sqrt{n}(\hat\theta-\theta^*)\dto\cN(0,\mathbf\Sigma),
\end{equation*}
as $n\to\infty$, where the asymptotic variance is given by $\mathbf\Sigma=\mathrm{Var}(\zeta+\xi)$ with 
\begin{align*}
	\zeta&=-H_g^{-1} h'(Z;\theta^*)/\sqrt\lambda\\
	\xi&=H_g^{-1}CH_d^{-1}\left[\nabla_{\psi}l_1(X;\psi^*)+\nabla_{\psi}l_2(G_{\theta^*}(Z);\psi^*)/\sqrt\lambda\right].
\end{align*}
\end{proof}



\subsection{Proof of Theorem \ref{thm:f_asy_normal}}\label{app:pf_f_asy_normal}
\begin{proof}
	We can show the asymptotic normality of $\hat\theta_f$ by the arguments similar to those in the proof of Theorem \ref{thm:asy_normal} where we replace $l_i$  by $l^f_i$ for $i=1,2$.
\end{proof}




\section{Proofs in Section \ref{sec:misspecify}}

\subsection{Proof of Theorem \ref{thm:d_asy_var_compare}}\label{app:pf_d_asy_var_compare}

We begin with a simple technical lemma.
\begin{lemma}\label{lem:sigma0}
	Let random vector $\tilde{X}=(1,X^\top)^\top$ and random variable $Y$. Suppose $\bbE(Y\tilde{X}\tilde{X}^\top)$ is positve definite. Then we have $$\bbE^{-1}(Y\tilde{X}\tilde{X}^\top)\bbE(Y\tilde{X})\bbE(Y\tilde{X})^\top\bbE^{-1}(Y\tilde{X}\tilde{X}^\top)=\Sigma_0,$$ where $\Sigma_0$ is a matrix whose first diagonal entry is 1 while all other entries are 0.
\end{lemma}
\begin{proof}
Let $\bbE(Y)=\alpha$, $\mu=\bbE(YX)$, and $V=\bbE(YXX^\top)$. We have
\begin{equation*}
	\bbE(Y\tilde{X}\tilde{X}^\top)=
	\begin{pmatrix}
		\alpha & \alpha\mu^\top\\
		\alpha\mu & V
	\end{pmatrix},\ 
	\bbE(Y\tilde{X})\bbE(Y\tilde{X})^\top=
	\begin{pmatrix}
		\alpha^2 & \alpha\mu^\top\\
		\alpha\mu & \mu\mu^\top
	\end{pmatrix}.
\end{equation*}
Let $k=\alpha-\mu^\top V^{-1}\mu$. Then, after some simplifications, we have
\begin{equation*}
	\bbE^{-1}(Y\tilde{X}\tilde{X}^\top)\bbE(Y\tilde{X})=
	\begin{pmatrix}
		\frac{1}{k}\left(\alpha-\mu^\top V^{-1}\mu\right)\\
		-\frac{\alpha}{k}V^{-1}\mu+\left(V-\mu\mu^\top/\alpha\right)^{-1}\mu
	\end{pmatrix}=
	\begin{pmatrix}
		1\\\mathbf{0}
	\end{pmatrix},
\end{equation*}
where $\mathbf{0}$ denotes a zero vector of the same dimension as $X$. Then the desired result follows.
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:d_asy_var_compare}]
We first explicitly compute the asymptotic variance of $\hat{\psi}$ and $\hat\psi_f$ for various $f$-divergences to obtain the results in Table \ref{tab:var_d}. 

For AGE, we first compute the derivatives of the discriminator loss
\begin{equation*}
	\nabla_\psi l_1(x;\psi)=-\frac{1}{1+e^{D_\psi(x)}/\lambda}\nabla_\psi D_\psi(x),\ \nabla_\psi l_2(x;\psi)=\frac{e^{D_\psi(x)}}{1+e^{D_\psi(x)}/\lambda}\nabla_\psi D_\psi(x);
\end{equation*}
\begin{equation*}
	\nabla^2_\psi l_1(x;\psi)=-\frac{1}{1+e^{D_\psi(x)}/\lambda}\nabla_\psi^2D_\psi(x)+\frac{e^{D_\psi(x)}/\lambda}{(1+e^{D_\psi(x)}/\lambda)^2}\nabla_\psi D_\psi(x)\nabla_\psi D_\psi(x)^\top,
\end{equation*}
\begin{equation*}
	\nabla^2_\psi l_2(x;\psi)=\frac{e^{D(x)}}{1+e^{D(x)}/\lambda}\nabla_\psi^2D_\psi(x)+\frac{e^{D_\psi(x)}}{(1+e^{D_\psi(x)}/\lambda)^2}\nabla_\psi D_\psi(x)\nabla_\psi D_\psi(x)^\top.
\end{equation*}
Then 
\begin{equation*}
	V_d=\bbE_{p_*}\left[\frac{p_\theta}{p_\theta+p_*/\lambda}\nabla_\psi D_{\psi^*} \nabla_\psi D_{\psi^*}^\top\right]-\left(1+\frac{1}{\lambda}\right)\bbE_{p_*}\left[\frac{p_\theta}{p_\theta+p_*/\lambda}\nabla_\psi D_{\psi^*}\right]\bbE_{p_*}\left[\frac{p_\theta}{p_\theta+p_*/\lambda}\nabla_\psi D_{\psi^*}\right]^\top
\end{equation*}
%where the second equality follows from Lemma \ref{}, 
and
\begin{equation*}
H_d=\bbE_{p_*}\left[\frac{p_\theta}{p_\theta+p_*/\lambda}\nabla_\psi D_{\psi^*} \nabla_\psi D_{\psi^*}^\top\right].
\end{equation*}

As supposed in the theorem, the first dimension of the parameter $\psi$ corresponds to the intercept, i.e., the first entry of $\nabla_\psi D_\psi(x)$ equals 1. By Lemma \ref{lem:sigma0}, we have 
\begin{equation*}
	\bbE_{p_*}^{-1}\Big[\frac{p_\theta}{p_\theta+p_*/\lambda}{\nabla_\psi D_{\psi^*}}^{\otimes2}\Big] \left(\bbE_{p_*}\Big[\frac{p_\theta}{p_\theta+p_*/\lambda}\nabla_\psi D_{\psi^*}\Big]\right)^{\otimes2}\bbE_{p_*}\Big[\frac{p_\theta}{p_\theta+p_*/\lambda}{\nabla_\psi D_{\psi^*} }^{\otimes2}\Big]=\Sigma_0.
\end{equation*}

Thus the asymptotic variance is given by 
\begin{equation*}
	\Sigma_d=\bbE_{p_*}^{-1}\left[\frac{p_\theta}{p_\theta+p_*/\lambda}{\nabla_\psi D_{\psi^*}}^{\otimes2}\right]-\Big(1+\frac{1}{\lambda}\Big)\Sigma_0.
\end{equation*}

Next, we compute the asymptotic variances of the discriminator of $f$-GANs for various $f$-divergences. To lighten the notation, throughout the remainder of this proof, we omit the subscript $\psi$ in $\nabla_\psi D_{\psi^*}$.

\medskip
\noindent
\textit{$f$-GAN-KL}

We recall from Table \ref{tab:fgan_loss} that the discriminator loss of $f$-GAN-KL is
\begin{equation*}
	L_k(\psi)=\bbE_{p_*}[l_1^f(X;\psi)]+\bbE_{p_\theta}[l_2^f(X;\psi)]=\bbE_{p_*}[-D_\psi(X)]+\bbE_{p_\theta}[e^{D_\psi(X)}].
\end{equation*}
Then we have 
\begin{equation*}
	H_k=\bbE_{p_*}\left[\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right]
\end{equation*}
\begin{equation*}
	\mathrm{Var}_{p_*}(\nabla_\psi l^k_1(X;\psi^*))=\bbE_{p_*}\left[\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right]-\bbE_{p_*}[\nabla D_{\psi^*}]\bbE_{p_*}[\nabla D_{\psi^*}]^\top
\end{equation*}
\begin{equation*}
	\mathrm{Var}_{p_\theta}(\nabla_\psi l^k_2(X;\psi^*))=\bbE_{p_*}\left[\frac{p_*}{p_\theta}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right]-\bbE_{p_*}[\nabla D_{\psi^*}]\bbE_{p_*}[\nabla D_{\psi^*}]^\top.
\end{equation*}
Hence the asymptotic variance of $\hat\theta_k$ is given by
\begin{equation*}
\Sigma_k=\bbE_{p_*}^{-1}\left[\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right] \bbE_{p_*}\left[\frac{p_\theta+p_*/\lambda}{p_\theta}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right] \bbE_{p_*}^{-1}\left[\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right]-\Big(1+\frac{1}{\lambda}\Big)\Sigma_0.
\end{equation*}

Then we compare $\Sigma_k$ with $\Sigma$ of AGE. Let random variable $\tilde{p}=p_\theta/(p_\theta+p_*/\lambda)$. Consider random vectors $\eta_1=\nabla D_{\psi^*}/\sqrt{\tp}$ and $\eta_2=\nabla D_{\psi^*}\cdot\sqrt{\tp}$. Note that $\Sigma_{d1}=(\bbE[\eta_2\eta_2^\top])^{-1}$ and $\Sigma_{k1}=(\bbE[\eta_1\eta_2^\top])^{-1} \bbE[\eta_1\eta_1^\top](\bbE[\eta_1\eta_2^\top])^{-1}$, where $\Sigma_{d1}$ and $\Sigma_{k1}$ denote the first terms in $\Sigma_d$ and $\Sigma_k$.
Then by Cauchy-Schwartz inequality in the matrix form \cite{tripathi1999matrix}, we know $\Sigma_{d1}\preceq\Sigma_{k1}$, where the equality holds if and only if $\tp=c$. By noting the definition of $\tp$, this leads to $(1-c)p_\theta=cp_*/\lambda$. By integrating both sides, we have $c=\lambda/(1+\lambda)$, that is, $p_\theta=p_*$, which never happens due to model mis-specification in Assumption \ref{ass:model_mis}. Therefore we have $\Sigma_d\prec\Sigma_k$.

\medskip
\noindent
\textit{$f$-GAN-RevKL}

We recall from Table \ref{tab:fgan_loss} that the discriminator loss of $f$-GAN-RevKL is
\begin{equation*}
	L_r(\psi)=\bbE_{p_*}[e^{-D_\psi(X)}]+\bbE_{p_\theta}[D_\psi(X)].
\end{equation*}
Similarly, the asymptotic variance of $\hat\theta_r$ is given by
\begin{equation*}
\Sigma_r=\bbE_{p_\theta}^{-1}\left[\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right] \bbE_{p_\theta}\left[\frac{p_\theta+p_*/\lambda}{p_*}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right] \bbE_{p_\theta}^{-1}\left[\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right]-\Big(1+\frac{1}{\lambda}\Big)\Sigma_0.
\end{equation*}
%Hence we have the asymptotic variance $V(\hat{D}_{f\rm{GANr}}(x))=\xi\Sigma_r\xi^\top$.

Write $\Sigma_{d1}=\bbE^{-1}_{p_\theta}\Big[\frac{p_*}{p_\theta+p_*/\lambda}\nabla D_{\psi^*} \nabla D_{\psi^*}^\top\Big]$. Let $\Sigma_{r1}$ denote the first term of $\Sigma_r$. Then by applying Cauchy-Schwartz inequality as in the KL case, we have $\Sigma_{d1}\preceq\Sigma_{r1}$ and hence $\Sigma_d\prec\Sigma_r$.

\medskip
\noindent
\textit{$f$-GAN-JS}

We recall from Table \ref{tab:fgan_loss} that the discriminator loss of $f$-GAN-JS is
\begin{equation*}
	L_j(\psi)=\bbE_{p_*}[\ln(1+e^{-D(X)})]+\bbE_{p_\theta}[\ln(1+e^{D(x)})].
\end{equation*}
Similarly, the asymptotic variance of $\hat\theta_j$ is given by
\begin{equation*}
\Sigma_j=\bbE_{p_\theta}^{-1}\bigg[\frac{p_\theta}{p_\theta+p_*}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\bigg] \bbE_{p_\theta}\bigg[\frac{p_\theta^2+p_*p_\theta/\lambda}{(p_\theta+p_*)^2}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\bigg] \bbE_{p_\theta}^{-1}\bigg[\frac{p_\theta}{p_\theta+p_*}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\bigg]-\Big(1+\frac{1}{\lambda}\Big)\Sigma_0.
\end{equation*}

Let $\eta_1=\frac{p_\theta}{p_\theta+p_*}\nabla D_{\psi^*}/\sqrt{\tp}$ and $\eta_2=\nabla D_{\psi^*}\cdot\sqrt{\tp}$. Then by applying Cauchy-Schwartz inequality similarly as above, we have $\Sigma_d\prec\Sigma_{j}$.

\medskip
\noindent
\textit{$f$-GAN-$H^2$}

We recall from Table \ref{tab:fgan_loss} that the discriminator loss of $f$-GAN-$H^2$ is
\begin{equation*}
	L_h(\psi)=\bbE_{p_*}[e^{-D_\psi(X)/2}]+\bbE_{p_\theta}[e^{D_\psi(X)/2}].
\end{equation*}
Similarly, the asymptotic variance of $\hat\theta_h$ is given by
\begin{equation*}
\Sigma_h=\bbE_{p_*}^{-1}\left[\sqrt{\frac{p_\theta}{p_*}}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right] \bbE_{p_*}\left[\frac{p_\theta+p_*/\lambda}{p_*}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right] \bbE_{p_*}^{-1}\left[\sqrt{\frac{p_\theta}{p_*}}\nabla D_{\psi^*}\nabla D_{\psi^*}^\top\right]-\Big(1+\frac{1}{\lambda}\Big)\Sigma_0.
\end{equation*}

Recall $\tilde{p}=p_\theta/(p_\theta+p_*/\lambda)$. We have $\sqrt{p_\theta/p_*}=\sqrt{\tp/(1-\tp)}$ and $(p_*+p_\theta)/p_*=1/(1-\tp)$.
Now we let $\eta_1=\nabla D_{\psi^*}/\sqrt{1-\tp}$ and $\eta_2=\sqrt{\tp}\nabla D_{\psi^*}$. Then by applying Cauchy-Schwartz inequality similarly as above, we have $\Sigma_d\prec\Sigma_{h}$.
\end{proof}



\subsection{Proof of Proposition \ref{prop:var_diff}}\label{app:pf_var_diff}
\begin{proof}
To lighten the notation, in this proof, we denote $d=\nabla_\psi D_{\psi^*}$.
For the KL divergence, we note that 
\begin{equation*}
	\Sigma_{k1}-\bbE_{p_*}^{-1}(dd^\top)=\bbE_{p_*}^{-1}(dd^\top)\bbE_{p_*}\bigg[\frac{p_*/\lambda}{p_\theta}dd^\top\bigg]\bbE_{p_*}^{-1}(dd^\top)=\Theta(1/\lambda)
\end{equation*}
\begin{equation*}
	\Sigma_{d1}-\bbE_{p_*}^{-1}(dd^\top)=\bbE_{p_*}^{-1}\bigg[\frac{p_\theta}{p_\theta+p_*/\lambda}dd^\top\bigg]\bbE_{p_*}\bigg[\frac{p_*/\lambda}{p_\theta+p_*/\lambda}dd^\top\bigg]\bbE_{p_*}^{-1}(dd^\top)=\Theta(1/\lambda),
\end{equation*}
which leads to $\|\Sigma_{k}-\Sigma_d\|=\Theta(1/\lambda)$.

For the reverse KL divergence, we have 
\begin{equation*}
	\Sigma_{r1}-\frac{1}{\lambda}\bbE_{p_\theta}^{-1}(dd^\top)=\bbE_{p_\theta}^{-1}(dd^\top)\bbE_{p_\theta}\bigg[\frac{p_\theta}{p_*}dd^\top\bigg]\bbE_{p_\theta}^{-1}(dd^\top)=\Theta(1)
\end{equation*}
\begin{equation*}
	\Sigma_{d1}-\frac{1}{\lambda}\bbE_{p_\theta}^{-1}(dd^\top)=\bbE_{p_\theta}^{-1}\bigg[\frac{p_*}{p_\theta+p_*/\lambda}dd^\top\bigg]\bbE_{p_\theta}\bigg[\frac{p_\theta}{p_\theta+p_*/\lambda}dd^\top\bigg]\bbE_{p_\theta}^{-1}(dd^\top)=\Theta(1),
\end{equation*}
which leads to $\|\Sigma_{r}-\Sigma_d\|=\Theta(1)$. Similarly, one can show $\|\Sigma_{j}-\Sigma_d\|=\Theta(1)$ and $\|\Sigma_{h}-\Sigma_d\|=\Theta(1)$.
\end{proof}




\section{Proofs in Section \ref{sec:well_specify}}

\subsection{Proof of Corollary \ref{cor:f_equiv}}\label{app:pf_f_equiv}
\begin{proof}
When the generated model is correctly specified, we have $p_*(x)=p_{\theta^*}(x)$, a.e. Then the optimal discriminator at the optimal generator is a constant function $D^*_{\theta^*}(x)=\ln (p_*(x)/p_{\theta^*}(x))=1$, a.e., which implies $\nabla_x D^*_{\theta^*}(x)=0$. Then $h'(z;\theta^*)=0$, a.e., so in the limiting distribution of $\hat\theta$ in Theorem \ref{thm:asy_normal}, $\zeta$ vanishes with probability 1. Hence the asymptotic variance of $\hat\theta$ becomes $\mathbf\Sigma=\mathrm{Var}(\xi)=H_g^{-1}C\Sigma_{d,\theta^*} C^\top H_g^{-1}$. We have 
\begin{equation*}
	H_g=\bbE[\nabla^2 l_g(\theta^*)]=\bbE[\nabla_\theta h'(Z;\theta^*)]=\bbE\left[s^*(G_{\theta^*}(Z))\nabla_\theta[\nabla_\theta G_{\theta^*}(Z)^\top\nabla_x D^*(G_{\theta^*}(Z))]\right]
\end{equation*}
and 
\begin{equation*}
	C=\nabla_\psi\bbE[h'_{D_{\psi^*}}(Z,\theta^*)]=\bbE\left[s^*(G_{\theta^*}(Z))\nabla_\theta G_{\theta^*}(Z)^\top\nabla_\psi\nabla_x D_{\psi^*}(G_{\theta^*}(Z))\right].
\end{equation*}
The scaling factors for various $f$-divergences at the optimal generator, with $r=e^{D_{\theta^*}^*(x)}=1$, is listed in the following table. Then $H_g^{-1}C$ is free of the $f$-divergence used. 
\begin{table}[h]
\vskip -0.1in
\centering
\caption{Optimal scaling factors for various $f$-divergences.}
\vskip 0.1in
\begin{tabular}{ccccc}
\toprule
$f$-divergence & KL & RevKL & 2JS & $H^2$\\\midrule
$s^*$ & 1 & 1 & 1/2 & 1/2\\
\bottomrule
\end{tabular}
\end{table} 

From Table \ref{tab:var_d}, considering $p_{\theta^*}=p_*$, all the asymptotic variances of the discriminator are simplified into 
\begin{equation*}
	\Sigma_{d,\theta^*}=\bigg(1+\frac{1}{\lambda}\bigg)\left(\bbE_{p_*}^{-1}\big[{\nabla_\psi D_{\psi^*}}^{\otimes2}\big]-\Sigma_0\right),
\end{equation*}
which again is free of the $f$-divergence used. Then by comparing $H_g,C,\Sigma_{d,\theta^*}$ with $H'_g,C',\Sigma'_{d,\theta^*}$ in the corollary statement, we complete the proof.
\end{proof}



\subsection{Proof of Corollary \ref{cor:gaus}}\label{app:pf_cor_gaus}
\begin{proof}
%According to Corollary \ref{cor:f_equiv}, AGE estimator $\hat\theta$ and $f$-GAN estimator $\hat\theta_f$ are asymptotically equivalent in this case, so we prove the result holds for $\hat\theta$, which directly implies that for $\hat\theta_f$. 
Similar to the proof of Corollary \ref{cor:f_equiv}, the asymptotic variance of $\hat\theta$ is $\mathbf\Sigma=H_g^{-1}C\Sigma_{d,\theta^*} C^\top H_g^{-1}$. 
Then it suffices to show $H_g^{-1}C\Sigma_{d,\theta^*} C^\top H_g^{-1}=(1+1/\lambda)\id_d$ in this case.
%When the generated model is correctly specified, i.e., $p_*(x)=p_{\theta^*}(x)$, a.e., then $D^*_{\theta^*}(x)=\ln (p_*(x)/p_\theta(x))=1$ a.e. Then $h'(z;\theta^*)=0$ a.e., so in the limiting distribution of $\hat\theta$ in Theorem \ref{thm:asy_normal}, $\zeta$ vanishes with probability 1. Hence the asymptotic variance becomes $\mathbf\Sigma=\mathrm{Var}(\xi)=H_g^{-1}C\Sigma_{d,\theta^*} C^\top H_g^{-1}$. 

Under this scenario, we have $\nabla_\theta G_\theta(z)=\id_d$, $\nabla_x D_\psi(x)=\psi_1$, and $\nabla_\psi D_\psi(x)=(1,x^\top)^\top$. Then $h'_{D_\psi}(\theta)=-e^{D_\psi(G_\theta(z))}\psi_1$. Then we have $H_g=-\bbE_{p_*}[\nabla_\theta\ln p_\theta(X)]=\id_d$, $C=(\mathbf{0},\id_d)$, and
\begin{align*}
	\Sigma_{d,\theta^*}&=\bbE_{p_*}^{-1}\left[\frac{p_{\theta^*}}{p_{\theta^*}+p_*/\lambda}{\nabla_\psi D_{\psi^*}}^{\otimes2}\right]-\Big(1+\frac{1}{\lambda}\Big)\Sigma_0=\Big(1+\frac{1}{\lambda}\Big)\left[\bbE_{p_*}^{-1}
	\begin{pmatrix}
		1 & x^\top\\
		x & xx^\top
	\end{pmatrix}
	-\Sigma_0\right]\\
	&=\Big(1+\frac{1}{\lambda}\Big)\left[
	\begin{pmatrix}
		1 & m_0^\top\\
		m_0 & m_0m_0^\top+\id_d
	\end{pmatrix}^{-1}
	-\Sigma_0\right]=\Big(1+\frac{1}{\lambda}\Big)
	\begin{pmatrix}
		m_0^\top m_0 & -m_0^\top\\
		-m_0 & \id_d
	\end{pmatrix}.
\end{align*}
Multiplication of them gives $\mathbf\Sigma=(1+1/\lambda)\id_d$, which completes the proof.
\end{proof}


\subsection{Proof of Corollary \ref{cor:localgan}}
For the purpose of analysis, we write down an algorithm analogous to Algorithm \ref{alg:localgan} in Algorithm \ref{alg:localgan*}, where $S(\hat\theta;x)$ is replaced by $S(\theta^*;x)$ and the gradient estimator is given by
\begin{equation}\label{eq:h_psi0}
	h_\psi(\theta)=\frac{1}{m}\sum_{i=1}^m \left[-\nabla_\theta S(\hat\theta;G_\theta(z_i))^\top\nabla_s D_\psi(S(\theta^*;G_\theta(z_i)))\right].
\end{equation}
For simplicity, let $\hat\theta_1$ be the output of Algorithm \ref{alg:localgan} (denoted by $\hat\theta_{\text{local}}$ in the main text) and $\hat\theta_0$ be the output of Algorithm \ref{alg:localgan*}, both with $T=O(n)$. 

{\centering
\begin{minipage}{.84\linewidth}
\vskip 0.1in
\begin{algorithm}[H]
\DontPrintSemicolon
\KwInput{Sample $\cS_n$, initial estimator $\hat\theta$, meta-parameter $T$}
Initialize $\theta_0=\hat\theta$\\
\For{$t=1,2,\dots,T$}{
True scores $s_i=S(\theta^*;x_i)$ for $i=1,\dots,n$\\
Generated scores $\hat{s}_i=S(\theta^*;G_{\theta_{t-1}}(z_i))$ for $i=1,\dots,m$\\
$\hat{\psi}_t=\argmin_{\psi\in\Psi}\big[\frac{1}{n}\sum_{i=1}^{n}\ln(1+e^{-D_\psi(s_i)}\lambda)+\frac{\lambda}{m}\sum_{i=1}^{m}\ln(1+e^{D_\psi(\hat{s}_i)}/\lambda)\big]$\\
$\theta_t=\theta_{t-1}-\eta {{h}_{\hat{\psi}_t}(\theta_{t-1})}$ for some $\eta>0$
}
\KwReturn{$\theta_T$}
\caption{Local GAN with optimal score}
\label{alg:localgan*}
\end{algorithm}
\end{minipage}
\vskip 0.1in
\par
}

We first prove two lemmas which show that $\hat\theta_0$ and $\hat\theta_1$ share the same asymptotic distributions.
\begin{lemma}\label{lem:pf_localgan1}
	Under conditions D1-D3, as $n\to\infty$, we have 
\begin{align}
	\frac{1}{n}\sum_{i=1}^n S(\hat\theta;x_i)&=\frac{1}{m}\sum_{i=1}^m S(\hat\theta;G_{\hat\theta_1}(z_i))+O_p(1/n),\label{eq:local_theta1}\\
	\frac{1}{n}\sum_{i=1}^n S(\theta^*;x_i)&=\frac{1}{m}\sum_{i=1}^m S(\theta^*;G_{\hat\theta_0}(z_i))+O_p(1/n).\label{eq:local_theta0}
\end{align}
\end{lemma}

\begin{proof}
Below we prove (\ref{eq:local_theta0}) for simplicity and (\ref{eq:local_theta1}) can be similarly proved.
We first show that $h_{\hat\psi_0}(\hat\theta_0)=O_p(1/n)$, where $\hat\psi_0$ is the solution of 
\begin{equation}\label{eq:psi_0}
	\min_{\psi}\left[\frac{1}{n}\sum_{i=1}^{n}\ln(1+e^{-D_\psi(S(\theta^*;x_i))}\lambda)+\frac{\lambda}{m}\sum_{i=1}^{m}\ln(1+e^{D_\psi(S(\theta^*;G_{\hat\theta_0}(z_i)))}/\lambda)\right].
\end{equation}
Adopting the same definitions as before, we have $\hat\delta'(\theta)=h_{\hat{D}}(\theta)-\nabla\hat L'(\theta)$ and $\hat\delta'=\sup_{\|\theta-\theta^*\|=O_p(1/\sqrt{n})}\|\hat\delta'(\theta)\|$. Then similarly to the arguments in the proof of Theorem \ref{thm:g_rate} and by noting (\ref{eq:linear_d}), we have $\hat\delta'=O_p(1/n)$. 

Suppose $L'(\theta)$ is $\ell_0$-smooth. Then we have
\begin{equation*}
	\hat L'(\theta_t) \leq \hat L'(\theta_{t-1}) - \eta h_{\hat\psi_t}(\theta_{t-1})^\top\nabla \hat L'(\theta_{t-1}) + \frac{\eta^2\ell_0}{2}\|h_{\hat\psi_t}(\theta_{t-1})\|^2.
\end{equation*}
Under the case where $\|h_{\hat\psi_t}(\theta_{t-1})\|^2\geq 2\hat\delta'^2$, we have
\begin{align*}
	-\eta h_{\hat\psi_t}(\theta_{t-1})^\top\nabla \hat L'(\theta_{t-1})&=-\eta h_{\hat\psi_t}(\theta_{t-1})^\top\left(h_{\hat\psi_t}(\theta_{t-1})+\hat\delta(\theta_{t-1})\right)\\
	&\leq \eta \left(-\|h_{\hat\psi_t}(\theta_{t-1})\|^2 +(\|h_{\hat\psi_t}(\theta_{t-1})\|^2+\|\hat\delta\|^2)/2\right)\\
	&=-\frac{\eta}{2}\left(\|h_{\hat\psi_t}(\theta_{t-1})\|^2-\hat\delta^2\right)\\
	&\leq -\frac{\eta}{4}\|h_{\hat\psi_t}(\theta_{t-1})\|^2,
\end{align*}
We note that
\begin{align*}
	\hat L'(\theta_t) &\leq \hat L'(\theta_{t-1}) - \frac{\eta}{4}\|h_{\hat\psi_t}(\theta_{t-1})\|^2 + \frac{\eta^2\ell_0}{2}\|h_{\hat\psi_t}(\theta_{t-1})\|^2\\
	&\leq \hat L'(\theta_{t-1}) - \frac{\eta}{8}\|h_{\hat\psi_t}(\theta_{t-1})\|^2,
\end{align*}
when $\eta<1/4\ell_0$, which can be satisfied with a sufficiently small learning rate.

By summing over $t=1,\dots,T$, we have  
\begin{equation*}
	\hat L'(\theta_T) \leq \hat L'(\theta_0) - 0.125 \eta \sum_{t=1}^T \|h_{\hat\psi_t}(\theta_{t-1})\|^2.
\end{equation*}
Note that $\hat L'(\theta)$ is lower bounded. Then we have $\sum_{t=1}^T \|h_{\hat\psi_t}(\theta_{t-1})\|^2 = O_p(1)$. Thus there exists $t$ in $\{0,\dots,T\}$ such that $\|h_{\hat\psi_t}(\theta_{t-1})\|^2 = O_p(1/T)=O_p(1/n)$. 

Otherwise there exists $t$ such that $\|h_{\hat\psi_t}(\theta_{t-1})\|<\sqrt{2}\hat\delta=O_p(1/n)$.% and hence we have $\|h_{\hat D}(\theta_{t-1})\|\to0$.

Therefore, by combining the two cases, we have $h_{\hat \psi_0}(\hat\theta_0)=O_p(1/n)$. 

Then by recalling the definition (\ref{eq:h_psi0}), we have
\begin{equation*}
	\frac{1}{m}\sum_{i=1}^m \left[-\nabla_\theta S(\hat\theta;G_\theta(z_i))^\top\right]\hat\psi_0=O_p(1/n),
\end{equation*}
which implies $\hat\psi_0=O_p(1/n)$. 

Also we have from the definition (\ref{eq:psi_0}) that
\begin{equation*}
	-\frac{1}{n}\sum_{i=1}^{n}\frac{1}{1+e^{D_{\hat\psi_0}(S(\theta^*;x_i))}/\lambda}\nabla_\psi D_{\hat\psi_0}(S(\theta^*;x_i))+\frac{1}{m}\sum_{i=1}^{m}\frac{e^{D_{\hat\psi_0}(S(\theta^*;G_{\hat\theta_0}(z_i)))}}{1+e^{D_{\hat\psi_0}(S(\theta^*;G_{\hat\theta_0}(z_i)))}/\lambda}\nabla_\psi D_{\hat\psi_0}(S(\theta^*;G_{\hat\theta_0}(z_i))) =0.
\end{equation*}
Note that $D_\psi(s)=\psi^\top s$, so $\nabla_\psi D_\psi(s)=s$. Further from the Taylor expansions
\begin{align*}
	\frac{1}{1+e^{D_\psi(s)}/\lambda}&=\frac{1}{1+1/\lambda}-\frac{1}{(1+1/\lambda)^2}\psi^\top s+o(\psi^\top s)\\
	\frac{1}{e^{-D_\psi(s)}+1/\lambda}&=\frac{1}{1+1/\lambda}+\frac{1}{(1+1/\lambda)^2}\psi^\top s+o(\psi^\top s),
\end{align*}
we obtain
\begin{equation*}
	-\frac{1}{n}\sum_{i=1}^n S(\theta^*;x_i)+\frac{1}{m}\sum_{i=1}^m S(\theta^*;G_{\hat\theta_0}(z_i))+O_p(1/n)=0,
\end{equation*}
which leads to (\ref{eq:local_theta0}).
\end{proof}

\begin{lemma}\label{lem:pf_localgan2}
	Under conditions D1-D3, as $n\to\infty$, we have $\hat\theta_1-\hat\theta_0=O_p(1/n)$. 
\end{lemma}

\begin{proof}
According to Lemma \ref{lem:pf_localgan1}, (\ref{eq:local_theta1})$-$(\ref{eq:local_theta0}) gives
\begin{equation*}
	\frac{1}{n}\sum_{i=1}^n S(\hat\theta;x_i)-\frac{1}{n}\sum_{i=1}^n S(\theta^*;x_i)=\frac{1}{m}\sum_{i=1}^m S(\hat\theta;G_{\hat\theta_1}(z_i))-\frac{1}{m}\sum_{i=1}^m S(\theta^*;G_{\hat\theta_0}(z_i))+O_p(1/n).
\end{equation*}
Since $\|\hat\theta-\theta^*\|=O_p(1/\sqrt{n})$, we have the following expansions
\begin{align*}
	\frac{1}{n}\sum_{i=1}^n S(\hat\theta;x_i)-\frac{1}{n}\sum_{i=1}^n S(\theta^*;x_i)&=\frac{1}{n}\sum_{i=1}^n H'(\theta^*;x_i) (\hat\theta-\theta^*)+O_p(1/n)\\
	\frac{1}{m}\sum_{i=1}^m S(\hat\theta;G_{\hat\theta_1}(z_i))-\frac{1}{m}\sum_{i=1}^m S(\theta^*;G_{\hat\theta_1}(z_i))&=\frac{1}{m}\sum_{i=1}^m H'(\theta^*;G_{\hat\theta_1}(z_i))(\hat\theta-\theta^*)+O_p(1/n)\\
	\frac{1}{m}\sum_{i=1}^m S(\theta^*;G_{\hat\theta_1}(z_i))-\frac{1}{m}\sum_{i=1}^m S(\theta^*;G_{\hat\theta_0}(z_i))&=\frac{1}{m}\sum_{i=1}^m \nabla_\theta S(\theta^*;G_{\theta}(z_i))|_{\hat\theta_0}(\hat\theta_1-\hat\theta_0)+O_p(1/n),
\end{align*}
where $H'(\theta;x)=\nabla_\theta S(\theta;x)$. 
Then we have
\begin{equation*}
	\hat\theta_1-\hat\theta_0=\left[\frac{1}{m}\sum_{i=1}^m \nabla_\theta S(\theta^*;G_{\theta}(z_i))|_{\hat\theta_0}\right]^{-1}\left[\frac{1}{n}\sum_{i=1}^n H'(\theta^*;x_i)-\frac{1}{m}\sum_{i=1}^m H'(\theta^*;G_{\hat\theta_1}(z_i))\right](\hat\theta-\theta^*)+O_p(1/n),
\end{equation*}
where we notice
\begin{equation*}
	\left[\frac{1}{m}\sum_{i=1}^m \nabla_\theta S(\theta^*;G_{\theta}(z_i))|_{\hat\theta_0}\right]^{-1}=O_p(1)
\end{equation*}
\begin{align*}
	\frac{1}{n}\sum_{i=1}^n H'(\theta^*;x_i)&=H(\theta^*)+O_p(1/\sqrt{n})\\
	\frac{1}{m}\sum_{i=1}^m H'(\theta^*;G_{\hat\theta_1}(z_i))&=\frac{1}{m}\sum_{i=1}^m H'(\theta^*;G_{\theta^*}(z_i))+O_p(1)(\hat\theta_1-\theta^*)\\
	&=H(\theta^*)+O_p(1/\sqrt{m})+O_p(1/\sqrt{n}),
\end{align*}
where $H(\theta)=\bbE_{p_*}[H'(\theta;X)]=\bbE_{p_*}[\nabla^2_\theta \ln p_\theta(x)]$. Hence we have $\hat\theta_1-\hat\theta_0=O_p(1/n).$
\end{proof}

\medskip
\begin{proof}[Proof of Corollary \ref{cor:localgan}]
To simplify the notation, throughout this proof, we let $\cI=\cI(\theta^*)$. 
According to Theorem \ref{thm:asy_normal}, Corollary \ref{cor:f_equiv}, and Lemma \ref{lem:pf_localgan2}, it suffices to show $H_g^{-1}C\Sigma_{d,\theta^*} C^\top H_g^{-1}=(1+1/\lambda)\cI$ for $\hat\theta_0$. % with the reverse KL divergence as the objective. 
We know that given $\theta$, the optimal discriminator in Algorithm \ref{alg:localgan*} is given by $D^*(s)=(\theta^*-\theta)^\top s$ up to higher order terms which do not affect the asymptotic variance. 
Then we have $\nabla_s D_{\psi}(s)=\psi$, $\nabla_\psi D_\psi(s)=s$, and $$h'_{D_\psi}(\theta)=-\nabla_\theta S(\theta^*;G_\theta(Z))^\top \nabla_s D_\psi(S(\theta^*;G_\theta(Z))).$$
Then we compute $H_g$, $C$ and $\Sigma_{d,\theta^*}$. It is easy to see $H_g=-\bbE_{p_*}[\nabla^2_\theta\ln p_\theta(X)]=\cI$. Let $p_*(s)$ be the distribution of $S(\theta^*;X)$ with $X\sim p_*(x)$. Then by noting that $\bbE_{p_*(s)}[S]=0$ and $\bbE_{p_*(s)}[SS^\top]=\cI^{-1}$ and that the discriminator does not have an intercept, we have
\begin{equation*}
	\Sigma_{d,\theta^*}=(1+1/\lambda)\bbE_{p*(s)}\big[\nabla_\psi D_{\psi^*}(S)\nabla_\psi D_{\psi^*}(S)^\top\big]=(1+1/\lambda)\cI^{-1}.
\end{equation*}
Also, we notice that
\begin{align*}
	\bbE_{p_z(z)}\Big[\nabla_\theta S(\theta^*;G_\theta(Z))^\top\Big]\Big|_{\theta^*}&=\nabla_\theta \bbE_{p_\theta(x)}\Big[S(\theta^*;X)\Big]\Big|_{\theta^*}\\
	&=\int\big[\nabla_\theta p_{\theta^*}(x)\big] S(\theta^*;x)^\top dx\\
	&=\int p_*(x)\big[\nabla_\theta \ln p_{\theta^*}(x)\big] S(\theta^*;x)^\top dx\\
	&= \bbE_{p_*(x)}\Big[S(\theta^*;X)S(\theta^*;X)^\top\Big]=\cI
\end{align*}
where the third equality is due to the fact that $p_*(x)=p_{\theta^*}(x)$, a.e., under the correctly specified case. Then we have
\begin{equation*}
	C=-\bbE_{p_z(z)}\Big[\nabla_\theta S(\theta^*;G_\theta(Z))^\top\Big]\Big|_{\theta^*}=-\cI.
\end{equation*}
Hence, we immediately know the asymptotic variance of $\hat\theta_0$ and also $\hat\theta_1$ is given by $H_g^{-1}C\Sigma_{d,\theta^*} C^\top H_g^{-1}=(1+1/\lambda)\cI$, which completes the proof.
\end{proof}



\section{Discussion on the regularity assumptions}\label{app:ass_eg}

In this section, we give a concrete example to illustrate the satisfaction of the regularity assumptions, as mentioned in Remark \ref{rem:ass_eg}. We restate the example here. Given a multivariate Gaussian as the real distribution on $\cX=\bbR^d$, i.e., $p_r(x)=\cN(\mu_0,\Sigma_0)$ where $\|\mu_0\|<\infty$ and $0<\|\Sigma_0\|<\infty$. Consider the generative model and discriminator satisfying the following:
\begin{itemize}\vspace{-0.05in}
\setlength{\itemsep}{1pt}
%\setlength{\parskip}{1pt}
\item Latent prior $p_z=\cN(0,\id_k)$ on $\cZ$.
%\item Additional random noise $\epsilon\sim p_\epsilon=\cN(0,I)$.
\item Linear generator class $\cG=\{G_\theta(z)=\theta_0+\theta_1z:\theta_0\in\bbR^{d},\theta_1\in\bbR^{d\times k},\|\theta_0\|\leq g_0,0<g_1\leq\|\theta_1\|\leq g_2\}$. Then $p_\theta(x)=\cN(\theta_0,\theta_1\theta_1^\top)$.
%\item Linear encoder class $\cE=\{Ex+e\epsilon:E\in\bbR^{k\times d},e\in\bbR^{k},  0<e_0\leq\|E\|\leq e_1,\|e\|\leq e_2\}$. Then $p_e(z|x)=\cN(Ex,e^2I_k)$.
\item Quadratic discriminator class $\cD=\{\psi_0+\psi_1^\top x+x^\top \psi_2 x: \psi_0\in\bbR, \psi_1\in\bbR^d, \psi_2\in\bbR^{d\times d}, 0<a_0\leq\|\psi_2\|\leq a_1,\|\psi_1\|\leq a_2,|\psi_0|\leq a_3\}$, where $a_i$'s depend on $g_i$'s, $\|\mu_0\|$, and $\|\Sigma_0\|$.
\end{itemize}%\vspace{-0.3cm}

Then the true and generated densities are given by
\begin{equation}\label{eq:eg_dist}
\begin{split}
	p_*(x)&=(2\pi)^{-\frac{d}{2}}[\det(\theta_1\theta_1^\top)]^{-\frac{1}{2}} e^{-\frac{1}{2}(x-\theta_0)^\top(\theta_1\theta_1^\top)^{-1} (x-\theta_0)}\\
	p_\theta(x)&=(2\pi)^{-\frac{d}{2}}[\det(\Sigma_0)]^{-\frac{1}{2}} e^{-\frac{1}{2}(x-\mu_0)^\top\Sigma_0^{-1} (x-\mu_0)}
\end{split}	
\end{equation}
%
Then the optimal discriminator is given by
\begin{equation}\label{eq:eg_D*}
	D^*_{\theta}(x)=\ln(p_*(x)/p_\theta(x))=\psi_0^*+{\psi_1^*}^\top x+x^\top \psi_2^* x
\end{equation}
where $\psi_0^*\in\bbR$, $\psi_1^*\in\bbR^{d}$, and $\psi_2^*\in\bbR^{d\times d}$ depend on parameters $\theta$.

% check conditions
We now verify the satisfaction of the assumptions on this example. According to (\ref{eq:eg_dist}), both $p_*$ and $p_\theta$ are multivariate Gaussians  whose covariances are bounded away from 0 and infinity. From (\ref{eq:eg_D*}) and the choice of $\cD$ we know that conditions \ref{ass:D_smooth} and \ref{ass:d_compact} hold. Because for each $D\in\cD$, we have $\nabla_x D(x)=\psi_1+2\psi_2 x$ and $\nabla_x^2 D(x)=2\psi_2$, and also the parameters are bounded, condition \ref{ass:D_bound} holds. 

Then we verify the uniform Lipschitz continuity of $\cD$ on any compact subset $K$ of $\cX$. Note there exists $B>0$ such that for all $x\in K$, we have $\|x\|\leq B$. Then for all $D\in\cD$ and  $x,x'\in K$,
\begin{align*}
	\|D(x)-D(x')\|&=\|(\psi_0+\psi_1^\top x+x^\top \psi_2 x)-(\psi_0+\psi_1^\top x'+{x'}^\top \psi_2 x')\|\\
	&\leq \|x^\top \psi_2 x-x^\top \psi_2 x'\|+\|x^\top \psi_2 x'-{x'}^\top \psi_2 x'\|+\|\psi_1^\top(x-x')\|\\
	&\leq (\|\psi_2x\|+\|\psi_2x'\|+\|\psi_1\|)\|x-x'\| \\
	&\leq (2a_1B+a_2)\|x-x'\|.
\end{align*}
The uniform Lipschitz continuity of $\{\nabla D:D\in\cD\}$ can be similarly obtained. 

For the envelope conditions, note that
\begin{equation*}
	\sup_{D\in\cD}|D(x)|=\sup_{\psi_0,\psi_1,\psi_2}\big|\psi_0 + \psi_1^\top x + x^\top \psi_2 x\big|\leq a_1\|x\|^2+a_2\|x\|+a_3,
\end{equation*}
\begin{equation*}
	\sup_{D\in\cD}\|\nabla D(x)\|=\sup_{\psi_1,\psi_2}\|\psi_1+2\psi_2x\|\leq 2a_1\|x\|+a_2.
\end{equation*}
Since Gaussian distributions have finite second moments, we know condition \ref{ass:envelope} holds. 

For condition \ref{ass:emp_envelop} we take the scaling factors of the reverse KL divergence as an example. Then 
\begin{equation*}
	h'(x,z;\theta)=\nabla_x D^*(G_\theta(z))^\top \nabla_\theta G_\theta(z).
\end{equation*}
Note that $\nabla_x D^*(G_\theta(z))$ and $\nabla_\theta G_\theta(z)$ are all linear in $x$. Also $\Theta$ is bounded. Hence the term within the expectation below is quadratic and we have %\tbm{(change to $\sup_{D\in\cD}$ instead of $D^*$)}
\begin{equation*}
	\bbE_{Z\sim p_z}\left[\sup_{\theta\in\Theta,D\in\cD}\big\|\nabla_x D(G_\theta(Z))^\top \nabla_\theta G_\theta(Z)\big\|\right]<\infty.
\end{equation*}



